Scalable Video Conferencing Using SDN Principles

Video-conferencing applications face an unwavering surge in traffic, stressing their underlying infrastructure in unprecedented ways. This paper rethinks the key building block for conferencing infrastructures -- selective forwarding units (SFUs). SFUs relay and adapt media streams between participants and, today, run in software on general-purpose servers. Our main insight, discerned from dissecting the operation of production SFU servers, is that SFUs largely mimic traditional packet-processing operations such as dropping and forwarding. Guided by this, we present Scallop, an SDN-inspired SFU that decouples video-conferencing applications into a hardware-based data plane for latency-sensitive and frequent media operations, and a software control plane for the (infrequent) remaining tasks, such as analyzing feedback signals. Our Tofino-based implementation fully supports WebRTC and delivers 7-210 times improved scaling over a 32-core commodity server, while reaping performance improvements by cutting forwarding-induced latency by 26 times.

==> sec/a1-ethics.tex <==
% !TEX root = ../p4-sfu.tex  

\section{Ethics}
\label{apx:ethics}

\noindent
The campus traces and the Zoom API data used in this study were anonymized with a one-way hash.
All data were inspected and sanitized by an authorized network operator to remove all personal data before being accessed by researchers.
In the packet traces, the media payloads have been removed as well before researchers gained access.
This study has been conducted with necessary approvals from our institution, including its Institutional Review Board (IRB).

==> sec/archive/5-data-plane-old.tex <==
\section{\sys{} Data Plane}
\label{sec:data-plane}

In this section, we describe \sys's data plane including its logic for its two main tasks: replication and rate adaptation.
% First, we discuss how SFU-based replication fundamentally differs from traditional multicasting (\S\ref{ssec:multicast-difference}). Second, we describe \sys's concrete design goals and the challenges in realizing them (\S\ref{ssec:design-goals-challenges}). Then, we describe our solutions to those challenges (\S\ref{ssec:replication}, \S\ref{ssec:suppression}, \S\ref{ssec:rewriting}) before finally describing our hardware prototype (\S\ref{ssec:hardware-prototype}). 
In addition, the data plane also ensures end-to-end SFU functionality by forwarding feedback packets, handling ARP, and responding to ICMP packets.
% sent to its dedicated IP.
% \joon{This last sentence does not feel important. cut?}

% The performance numbers in this section have been computed assuming meetings with between 3 to 10 participants with everyone sending video and audio at all times totaling a data rate of up to 3Mbps.

\subsection{SFU Media Replication vs. Multicasting}
\label{ssec:multicast-difference}

Traditional network multicasting was designed for one-to-many distribution where receivers request to join a multicast group, and routers replicate and forward packets accordingly.
In contrast, VCA SFUs have unique replication challenges that differ from traditional multicast models:
\begin{itemize}[leftmargin=*]
    \item \textbf{Per-Receiver Adaptation:} SFUs must dynamically adjust video quality per receiver, as opposed to IP multicast where every receiver receives the same stream.
    \item \textbf{Unicast Destinations:} Most real-world deployments rely on unicast-only networks (e.g., the public Internet, enterprise networks) where native IP multicast is unavailable.
\end{itemize}
SFU replication introduces significant complexity when mapped onto hardware replication engines (e.g., the Tofino's Packet Replication Engine (PRE)). While such replication engines are optimized for fast, parallel replication---offering significant improvement over sequential replication (e.g., in software)---their resources (e.g., maximum number of replication trees) are inherently limited and their flexibility (e.g., ability to \emph{prune} unneeded branches of multicast trees) inherently constrained, rendering such an endeavor a challenging one\jrex{very long sentence that is hard to parse}.

\subsection{Design Goals and Challenges}
\label{ssec:design-goals-challenges}

To efficiently support SFU-based media replication in hardware, our design must achieve the following goals while addressing the related challenges.

\boldpara{Scalable Media Replication.}
To achieve significant improvement in scalability over software-based SFUs, \sys{} relies on hardware-accelerated replication of media streams so that thousands of concurrent senders and meetings can be supported. However, because the number of multicast trees on hardware is limited due to resource constraints, \sys{} must use careful tree-aggregation techniques to fully leverage the switch’s high bandwidth.
\sys{} also needs to preserve the SFU’s rate-adaptation functionality by delivering one or more SVC layers to receivers based on the layer-selection algorithm. \sys{} must do the above while only creating packet replicas that are actually needed downstream---thereby avoiding wasteful over-replication. Since hardware-based multicast engines are not optimized for such use cases, identifying mappings between VCA entities (meetings, participants, senders) and replication tree entities (root, level 1 node, level 2 node), that ensure both correctness and efficiency, is challenging. We solve this by constructing three different types of efficient replication trees and migrating meetings among them dynamically (\S\ref{ssec:replication}).

% \boldpara{Scalable Packet Replication.} To achieve significant improvement in scalability over software-based SFUs, \sys{} needs to enable efficient replication of media streams such that thousands of concurrent senders and meetings can be supported without overwhelming network resources. However, while hardware-accelerated replication improves efficiency, since the number of multicast trees is inherently limited, \sys{} requires careful tree-aggregation techniques.

% \boldpara{Efficient Bandwidth Utilization.} To take full advantage of the hardware's high bandwidth (e.g., 6.4 Tbps on the Tofino), \sys{} should only create replicas that are actually consumed downstream. \joon{"take full advantage" means you want to fully use the bandwidth. But then you say you want to limit the usage by limiting downstream? I guess you mean.. efficiently use the bandwidth (so that other flows can take advantage?)} Aggregating multicast trees indiscriminately would create numerous unneeded replicas that need to be dropped, wasting egress bandwidth. Instead, \sys{} should dynamically prune multicast branches to \emph{suppress} the generation of unneeded replicas in the first place.

% \boldpara{Support for Rate Adaptation.} To preserve the SFU's functionality, \sys{} should deliver one or more SVC layers to receivers based on the decisions of the layer-selection algorithm that change over the course of the meeting. One could naively create a separate multicast tree per layer to support this; however, this quickly becomes unscalable, necessitating more sophisticated tree management techniques.

\boldpara{Transparent Rate Adaptation.} \sys{} should also ensure that quality layers dropped due to rate adaptation are not misinterpreted by receivers as network-induced packet loss, since that would trigger unnecessary retransmission requests, defeating the purpose of rate adaptation. Dropping quality layers \emph{transparently} to receivers requires rewriting the media stream's sequence numbers to maintain a seemingly continuous stream, which is challenging and even impossible to achieve perfectly when intentional drops coincide with network-induced loss and reordering (\S\ref{ssec:rewriting}).

% \boldpara{Dynamic Meeting Management.} \sys{} must handle frequent joins, leaves, and adjustments of quality levels. Efficiently updating replication structures in response to these changes, without causing excessive control overhead or introducing latency, is critical for seamless operation, but challenging due to the constraints of the hardware.

\subsection{Media Replication in Scallop}
\label{ssec:replication}
\sata{Trying to merge 6.3 and 6.4 currently.}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{fig/trees_without_rate_adaptation.pdf}
    \caption{Construction of progressively more efficient trees for SFU media replication by aggregating meetings and leveraging dynamic branch-pruning.}
    \label{fig:replication-trees}
\end{figure}

In this subsection, we discuss replication-tree designs for meetings that do not require rate adaptation.
%In the next subsection, we discuss how we incorporate rate adaptation.

\boldpara{Hardware replication capabilities.}
Networking hardware natively supports packet replication, but implementation details vary by platform. Generally, a replication engine manages a finite number of replication trees ($\mathcal{T}$), where each tree has a root node that replicates packets through multiple hierarchical levels before reaching leaf nodes mapped to egress ports. The maximum number of level-1 nodes far exceeds $\mathcal{T}$, and each subsequent level scales accordingly to maintain the tree structure. Many hardware-based replication engines also support \emph{pruning}, where packet replication is dynamically \emph{suppressed} based on pre-configured conditions set by the control plane and evaluated in the data plane.
Since our prototype is implemented on the Tofino, which supports two-level trees with pruning at both levels, we design our solutions considering these properties, without sacrificing general applicability.

\boldpara{Strawman.}
Due to the absence of prior work on leveraging hardware-based multicasting for SFU media replication, we had to systematically explore the design space of solutions. Our main challenge is mapping VCA entities (meetings, senders, receivers) onto the replication tree hierarchy (root, level-1 nodes, level-2 nodes). A straightforward approach, illustrated in Figure~\ref{fig:replication-trees}(a), assigns each media stream to a separate replication tree, where the sender (e.g., participant 1 in a meeting with three participants) is the root, the receivers (participants 2 and 3) are level-1 (L1) nodes, and their egress ports are level-2 (L2) nodes. While functional, this approach limits the system to $\mathcal{T}$ concurrent senders, creating a bottleneck and preventing full utilization of the hardware’s high bandwidth (e.g., 6.4 Tbps on Tofino).

\boldpara{Aggregating all senders in a meeting.} 
In Figure~\ref{fig:replication-trees}(b), we present a more efficient approach where all participants of a meeting are aggregated into a single tree. Here, the root represents the meeting, L1 nodes represent participants (whether sending, receiving, or both), and L2 nodes map each L1 node to its respective egress port. This design offers two key advantages over the strawman approach:
(1) Instead of supporting $\mathcal{T}$ \emph{individual senders}, the system now supports $\mathcal{T}$ \emph{meetings}; and
(2) For meetings with $\mathcal{N}$ participants (each sending and receiving), the strawman requires $\mathcal{N}(\mathcal{N}-1)$ L1 nodes per meeting, whereas our design requires only $\mathcal{N}$. However, a key limitation arises: when a sender transmits a packet, the root replicates it to all participants, including the sender, resulting in unnecessary bandwidth usage. To mitigate this, we leverage pruning at L2 to prevent replication to the sender.

\boldpara{Aggregating multiple meetings.}
While the previous design is already highly efficient, we can further optimize it to completely eliminate the possibility that the replication module becomes the performance bottleneck instead of the switch’s bandwidth. As illustrated in Figure~\ref{fig:replication-trees}(c), we achieve this by aggregating multiple meetings into a single replication tree. This approach still requires $\mathcal{N}$ L1 nodes per meeting, but now the system can support $m\mathcal{T}$ concurrent meetings, where $m$ is the number of meetings combined into one tree. The key challenge in this design is that packets from one meeting would, by default, be replicated to participants from other meetings at L1. To prevent this, we apply pruning at L1, ensuring that only participants belonging to the same meeting receive the packet. Pruning at L2 remains responsible for preventing the sender from receiving its own packet. We empirically verify that this design---which we call the non-rate-adapted (NRA) design---is also the most efficient design possible on the Tofino, with $m$=$2$ (\S\ref{ssec:hardware-prototype}).

\boldpara{Two-party meetings.}
While optimizing resource utilization for multi-party meetings is at the heart of designing an efficient SFU, two-party meetings are quite common ($60\%$ meetings in our campus dataset). Since two-party meetings do not require replication, we further optimize our design by not constructing replication trees for such meetings and treating the sender's media stream as unicast.
\joon{importance of this paragraph seems low. cut candidate.}

\boldpara{Addressing replicated packets.}
Unlike traditional multicast, where all replicas share the same source and multicast destination, an SFU must send each packet to a specific unicast receiver while preserving the semantics of a WebRTC-compliant split-proxy design. To achieve this, \sys{} rewrites packet headers in the egress pipeline, setting the SFU as the source and the receiver’s unicast address as the destination, before forwarding it to the correct port.

\subsection{Support for Rate Adaptation}
\label{ssec:suppression}

\boldpara{Challenge.}
\sys{} performs rate adaptation by selectively replicating SVC layers to receivers (\S\ref{ssec:svc-analysis-and-layer-selection}). With $L_1T_3$, three qualities are possible: low, mid, and high. The need to support multiple quality levels complicates the design of efficient replication trees due to the hardware's pruning constraints. Since replication trees are managed by the control plane, we can only update them infrequently (e.g., when participants join/leave or network conditions change), rather than per-packet, to maintain scalability. Meanwhile, packets can only carry limited switch-internal metadata to indicate which multicast branches should be pruned. As a result, we can either prune branches for a subset of participants or a subset of SVC layers for a packet---but not both simultaneously.

\boldpara{Receiver-specific rate adaptation.}
If the layer-selection algorithm assigns the same quality mode to a receiver across all senders---a common scenario we term receiver-specific rate adaptation---we address the aforementioned challenge as follows.
We retain our efficient NRA design but use separate replication trees for each quality level. For example, for $m$ rate-adapted meetings using $L_1T_3$, we create three distinct replication trees, each corresponding to a different quality level. The tree for the \emph{low} quality mode includes all participants from all $m$ meetings as L1 nodes. The trees for the \emph{mid} and \emph{high} quality modes contain only participants receiving the middle and the highest layer, respectively. With $t$ quality layers (where $t$=$3$ for $L_1T_3$), this design supports $m\mathcal{T}/t$ meetings while requiring up to $t\mathcal{N}$ L1 nodes. We refer to this as the Rate-Adapted Receiver (RA-R) design.

\boldpara{Sender-dependent rate adaptation.}
When a receiver’s quality mode varies across different senders (i.e., rate adaptation is sender-dependent), the best we can achieve is aggregating two senders (and their corresponding receivers) per quality level into a single replication tree. This design, called Rate-Adapted Sender-Receiver (RA-SR), supports $2\mathcal{T}/t\mathcal{N}$ meetings while consuming up to $2\mathcal{T}$ L1 nodes.

\boldpara{Migrating between replication-tree designs.}
Since rate adaptation is not always required, and even when required it may not be sender-dependent, we design the switch agent to dynamically migrate meetings between NRA, RA-R, and RA-SR modes as needed. This maximizes the utilization of the replication engine, ensuring that the bottleneck remains the switch’s bandwidth rather than replication capacity. To avoid meeting disruptions during migration, we: (1) create a new replication tree for the migrated meeting, (2) update data plane rules to redirect packets to the new tree, and (3) deallocate the old replication tree.

\subsection{Transparent Rate Adaptation}
\label{ssec:rewriting}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\columnwidth]{fig/seqnum_rewriting.pdf}
    \caption{Rewriting sequence nos. for rate adaptation.}
    \label{fig:seqnum-rewrite}
\end{figure}

\boldpara{Maintaining transparency to receiver.}
Since WebRTC assumes a P2P architecture, receivers expect a continuous, unmodified stream directly from the sender. However, SFUs performing rate adaptation suppress certain packets (in fact, with SVC, they suppress entire quality layers containing multiple packets) to match network conditions, creating gaps in RTP sequence numbers that could be misinterpreted as network loss, triggering unnecessary retransmissions. To maintain the illusion of a direct stream, \sys{} rewrites sequence numbers in a streaming fashion to mask intentional gaps, using limited hardware memory.

\boldpara{Rewriting in the absence of network loss.}
First, we consider a lossless and reorder-free network where gaps in sequence numbers arise solely from pruning during replication for rate adaptation. To handle these, we maintain a Stream Tracker hash table in the data plane, storing the \emph{last rewritten sequence number} per active stream (Figure~\ref{fig:seqnum-rewrite}). Each stream is uniquely identified by its sender’s and receiver’s addresses and SSRC. When the first packet from a newly tracked stream arrives, we store its sequence number; when subsequent packets from the stream arrive, we increment this value by $1$ and replace the packet's sequence number with it, ensuring continuity. Using its knowledge of rate-adapted active streams, the control plane computes a unique unused hash for a new stream it wants to track and installs it as a rule in the \emph{Stream Index} table, preventing hash collisions and efficiently reusing indices to optimize memory usage.

\boldpara{Rewriting in the presence of loss and reordering.}
Rewriting sequence numbers becomes increasingly challenging as network loss and reordering rates rise. The two main challenges arise when we observe: (1) large gaps in sequence numbers --- it is unclear how many frames were intentionally suppressed versus lost in transit, and (2) severely reordered packets -- An old packet arrives long after its \emph{offset} (difference between the original and the rewritten sequence numbers) was last tracked. To handle (1), we update the offset conservatively to ensure that no sequence number is ever repeated, regardless of future packet arrival order. For (2), we adjust the offset if safe; otherwise, we drop the packet, since the receiver is likely to have triggered a retransmission anyway. Under no circumstance do we allow repeated sequence numbers, as this would break the decoder’s state and freeze the media stream. If our heuristic miscalculates, it leaves a gap, triggering retransmission and causing some overhead. Multiple implementations of the above  heuristic are possible, with different trade-offs between accuracy, complexity, and state. Below, we briefly describe our most accurate heuristic.

We assume the control plane, via match-action tables, provides us with: (1) Frame-skip cadence (e.g., every third frame is suppressed), and (2) An estimate of minimum packets per frame (a more accurate estimate reduces overhead; default is 1). Each packet contains, in its headers, its frame number, original sequence number, quality layer, and a marker indicating if it’s the first, last, or an intermediate packet of its frame. The algorithm expands the Stream Tracker table to track the following per-stream state: maximum observed frame number ($\mathcal{F}_{max}$), the starting and highest sequence numbers of $\mathcal{F}_{max}$, a boolean value indicating whether the last frame's end marker was observed, the highest suppressed frame number, and the sequence number offset. Based on extracted packet data and stored state, the algorithm classifies packets into five cases and performs the following actions:
\begin{enumerate}[leftmargin=*]
    \item First packet in stream: Initialize state.
    \item Same frame as last observed: Update state, apply offset.
    \item Next consecutive frame: Update state, apply offset.
    \item Skipped frames: Compute, or conservatively estimate, how many packets were suppressed and adjust the offset.
    \item Old frame: If possible, apply a safe offset; otherwise, drop the packet to prevent sequence number duplication.
\end{enumerate}
Cases (1) to (3) are straightforward and trigger only state updates. In cases (4) and (5), we ensure that sequence numbers remain continuous and never repeat, even if this means introducing gaps and triggering retransmissions. This approach maintains smooth functionality with minimal overhead.
\joon{okay, I gave up at some point. Too much technical detail for me. Is this very Tofino-specific? If yes, not great. But.. is there any way to make a reviewer interested in learning this? Would it be useful for other use cases or in other contexts?}

\subsection{Hardware Prototype}
\label{ssec:hardware-prototype}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{fig/tofino_pre.pdf}
    \caption{Tofino's Packet Replication Engine (PRE).}
    \label{fig:tofino-pre}
\end{figure}

In this subsection, we describe how we implement the efficient replication and transparent rate adaptation techniques described earlier, on the Tofino.

\boldpara{Background on Tofino PRE.}
The PRE is a specialized hardware block in Tofino designed for efficient multicast through a hierarchical, three-level structure (called a \emph{multicast group} or a \emph{multicast tree}) managed by the control plane (Figure~\ref{fig:tofino-pre}). When the data plane assigns a multicast group ID (MGID) to an incoming packet, the PRE replicates the packet in two steps: the root replicates it to L1 nodes, which then replicate it to L2 nodes, which then direct the replicas to specific egress ports. The PRE can support up to 64K multicast trees and a total of 16.8M ($2^{24}$) L1 nodes.
Tofino's PRE also supports dynamic pruning of branches (red arrows in Figure~\ref{fig:tofino-pre}) using L1- and L2-exclusion IDs (XIDs).
% \joon{okay, some background on this Tofino PRE. This seems to come too late.}

\boldpara{Configuring the PRE.}
The switch control plane configures the PRE at runtime by first creating L1 nodes, each identified by a \emph{node ID} (unique across the PRE), \emph{replication ID} or RID (unique across one multicast tree), and \emph{egress port} (unique across one RID in a tree). The control plane then defines multicast trees, each with a unique MGID and an associated set of L1 nodes. Each L1 node is assigned an L1 XID and a flag indicating whether pruning (via the XID) is enabled. Additionally, the control plane maps each L2 XID to a specific subset of the switch's egress ports. The data plane invokes the PRE by assigning the packet's MGID, L1 XID, and RID--L2 XID pair in the ingress pipeline. We implement aggregated trees by setting L1-XID=1 for the participants of the first meeting and L1-XID=2 for those of the second, and then setting the correct one (L1-XID 2 for packets of meeting 1 and vice-versa) in the data plane. We prevent copies from being created for the sender by setting the packet's RID to the RID of the sender's node and it's L2-XID to its egress port. We identify replicated packets from the same sender uniquely in the egress pipeline by their RIDs (up to 65,536 per tree) and set the destination addresses accordingly.

\boldpara{Per-stream state.} The egress pipeline stores seven hash tables, always accessed in order, to enable sequence number rewriting on the Tofino. Each active rate-adapted stream maintains state across all 7 tables. Since the indices are managed by the control plane ensuring zero hash collisions and immediate cleanup when the stream ends, all cells in these tables can be used, allowing up to 65,536 concurrent streams.

% \boldpara{Deep parsing to identify packet type.}
% After parsing the Ethernet, IP, and UDP headers, we use the destination IP and port numbers to determine whether the packet is destined for the SFU. If so, we \emph{lookahead} into the first $4$ bits of the UDP payload to determine whether the packet resembles an RTP or an RTCP packet. If the packet is an RTP media packet or an RTCP sender report, we mark it for replication; otherwise, we forward it.
% Rate adaptation in SVC works by dropping packets that correspond to the higher quality layers of an AV1 media stream, as needed. Determining what quality layer a packet belongs to requires parsing into the RTP \emph{header extensions} beyond the RTP header, identifying the header extension corresponding to the AV1 protocol (if present), and parsing the AV1 header\footnote{We implement a Wireshark plugin to parse RTP header extensions to identify and display AV1 headers which we will open-source, along with all of our other source code, pertaining to both the control and data planes.} to extract its \emph{dependency template ID}, which when combined with the control plane's knowledge of the mapping between dependency templates and quality layers, tells us the quality layer of the packet itself. Parsing deep into the RTP header extensions to find the AV1 header requires handling variable-length and variable-position headers which is tricky because the P4 parser on Tofino relies on a largely static parse graph. We solve this by (i) implementing a \emph{depth-aware} parsing tree for the RTP header extensions, where for every depth in the tree, we have a \emph{landing state} that determines---using the \emph{lookahead} function---what type of header element (one-byte header, two-byte header, or padding) comes next, and (2) using the Tofino's \emph{ParserCounter} feature to track whether there are header bytes left to parse.
\joon{I think most of content in section 6.6 are not needed. I doubt anyone much care about this level of details, especially post-PhDs. }

==> sec/archive/arch1.tex <==
% !TEX root = ../p4-sfu-nsdi24.tex  

\section{Rethinking Video-Conferencing Infrastructure}
\label{sec:arch}

To provide an intuition for a disaggregated architecture of video-conferencing systems and the design of a switch-based SFU, we first discuss the detailed operation of a SFU and draw analogies to conventional packet-processing systems (\textsection\ref{ssec:arch:sfu-pkt-proc}) before detailing a control- and data-plane split inspired by SDN principles (\textsection\ref{ssec:arch:div-labor}).

\subsection{SFUs as Packet Processors}
\label{ssec:arch:sfu-pkt-proc}

SFUs perform two main tasks: (1) media forwarding and (2) rate adaptation (see Figure~\ref{fig:call-arch}).
Both tasks have striking similarities to traditional packet-processing tasks.

\noindent
\textbf{Media Forwarding in SFUs.}~%
%
Each media stream (audio or video) originates at a single participant and needs to be forwarded to all other participants.
Traditionally, this functionality has been performed in mixers (sometimes referred to as MCUs) which decode and re-encode the media streams to combine them into a single stream that is then forwarded to all participants.
This however, requires (1) decrypting all incoming packets, (2) decoding the media, (3) re-encoding it, and (4) encrypting it again which is computationally costly given the number of streams and their scaling properties (cf. \S\ref{ssec:provisioning-sfus}) and also introduces additional latency.
As a result, SFUs operate on packets rather than the actual media which is the key enabler for our work.

Analyzing Zoom packet traces collected on our campus, we observed that Zoom's SFUs do not perform any modification of the packets; they do not change header fields, do not translate sequence numbers, nor do they change the packet's encrypted payload in any way.
The same results have been reported in~\cite{michel:passive-measurement-zoom} where this insight is used to infer the number of participants in a given meeting.
Consequently, the forwarding operation of a SFU reduces to replicating a packet $N-1$ times for a meeting with $N$ participants and sending the resulting $N-1$ packets to the respective participants.

\noindent
\textbf{Rate Adaptation in SFUs.}~%
%
Taking into consideration that SFUs do not modify packet headers or packet payloads, the question remains how SFUs are even able to modify the quality (and consequently the bitrate) of a media stream for a specific downstream participant.
To understand this rate adaptation mechanism from the network perspective, we again collected packet-level traces of Zoom traffic in our campus network which we analyzed using the methods and tools presented in~\cite{michel:passive-measurement-zoom}.

We now show a real-world meeting with 19 participants on our campus interconnected through a Zoom SFU that took place in May 2022.
Figure~\ref{fig:kbits-per-stream} shows an example of a participant's outgoing video stream and the corresponding incoming streams at two other participants.
Time zero denotes the start of the meeting at which the sending participant starts transmitting a low-bitrate video stream which then increases in bitrate at around 20 seconds into the meeting.
Presumably in response to constrained downlink capacity, the SFU then reduces the bitrate forwarded to participant 12 (at around 110s) and the bitrate forwarded to participant 17 (at around 200s), respectively.

Zoom uses the Real-Time Transport Protocol (RTP)~\cite{rtp-rfc} encapsulated in custom, proprietary headers over UDP to transmit media~\cite{michel:passive-measurement-zoom}.
The RTP header carries a sequence number and various extension fields in each packet that is not being changed by Zoom's servers during forwarding.
As a result, we can exactly specify which packets are forwarded to a given participant by the SFU and which are not.
% We further observed that Zoom's RTP packets carry various RTP extension headers.
One header extension field carries a three-Byte value that appears to be a bit mask.
The packets in the outgoing media streams typically carry between two and six different values for this field across their packets which we for now denote as the \emph{packet type}.
We observe that the SFU only forwards either all or a strict subset of these packet types to a given participant; sometimes, this subset changes during the meeting.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\columnwidth]{fig/kbits-per-stream-1}
    \caption{Forwarded bytes of a single video stream to two separate participants in a Zoom meeting.}
    \label{fig:kbits-per-stream}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\columnwidth]{fig/kbits-per-layer-1}
    \caption{Forwarded bytes per scalability layer of a single video stream to a single participant in a Zoom meeting.}
    \label{fig:kbits-per-layer}
\end{figure}

Figure~\ref{fig:kbits-per-layer} shows the bit rate of the same media stream as previously shown broken down by packet type.
We can see that the adaptation of the media stream received by participant 17 around second 200 is achieved by changing the set of packet types forwarded to this client.
This is consistent with previous observations that Zoom uses Scalable Video Coding (SVC) or Simulcast~\cite{michel:passive-measurement-zoom,how-zoom-works, w3c:webrtc-svc, schwarz:svc-overview} and leverages this field to indicate to the SFU which layer of a scalable stream the respective packet carries.
It is common to encode the type of scalability layer in the RTP header~\cite{schwarz:svc-overview} which is transmitted in clear text; 
similar header extensions exist, for example, for the AV1 codec~\cite{av1, av1-rtp}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\columnwidth]{fig/sfu-operation.pdf}
    \caption{Media-Forwarding Operation of a SFU using SVC.}
    \label{fig:sfu-operation}
\end{figure}

The mechanism behind SVC is illustrated in Figure~\ref{fig:sfu-operation}.
Here, the SFU relays a media stream in a four-party meeting where one participant receives a reduced frame-rate stream (15 fps instead of 30 fps) which is achieved by dropping every other frame.
Additionally, media is packetized in such a way that scalability layers do not cross packet boundaries.
The letters A and B here denote the two different scalability layers, a base layer (A) and an enhancement layer (B) which depends on the base layer, as denoted by the black arrows.
We conclude that if SVC (or the related technology, Simulcast~\cite{lin:gso-simulcast}) is used, adapting a media stream reduces to forwarding a clearly defined and correspondingly labeled subset of packets to a given participant.

\subsection{Data Plane Programmability}
\label{ssec:arch:data-plane-prog}

Despite the similarities with conventional packet processing, traditional fixed-function network devices operate on a limited set of headers (e.g., Ethernet, IP, and MPLS) and are therefore not able to process the relevant headers and metadata fields in video-conferencing traffic.
Newer-generation devices, however, offer programmable packet parsers and reconfigurable processing pipelines, enabling network operators to define custom protocols and forwarding logic~\cite{michel:prog-data-plane}.
The most prominent example of such a device architecture is the Protocol-Independent Switch Architecture (PISA)~\cite{bosshart:sdn-chip}.
A PISA switch consists of a programmable parser which can support arbitrary protocols using a state-machine abstraction, a pipeline of match-action tables that can match header fields and perform actions on the packet (e.g., rewriting a field or performing basic calculations) in algorithmic logical units (ALUs), and a programmable deparser that reassembles the packet for transmission.
A popular language for the programming of such switches and other data-plane devices (e.g., SmartNICs or FPGAs) is P4~\cite{bosshart:p4}.
Many switches additionally offer a configurable packet-replication engine (PRE) that can replicate packets based on the match-action pipeline's state to, for example, realize multicast.
Among other platforms, such as FPGAs and certain SmartNICs, PISA switches allow us to efficiently implement selective forwarding based on parsed non-standard headers (e.g., the RTP extension fields) and to replicate or drop packets based on the same criteria in the PRE.

\subsection{Division of Labor}
\label{ssec:arch:div-labor}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{fig/arch.pdf}
    \caption{P4 SFU Architecture.}
    \label{fig:arch}
\end{figure}

% \begin{table}[t]
%     % data and analysis in: /Users/olli/src/research/webrtc-analysis/data/pkt_types
%     \centering
%     \footnotesize
%     \begin{tabular}{l|rrr|rr} 
%         % \hline
%         \textbf{Protocol/Type} & \textbf{Packets} & \textbf{Pct.} & \textbf{Per sec.} & \textbf{Kilobytes} & \textbf{Pct.} \\
%         \hline
%         RTP & 46,102 & 87.43 & 144.07 & 26,606 & 98.28 \\
%          - Audio & 16,001 & 30.34 & 50.00 & 2,287 & 8.45 \\
%          - Video & 30,101 & 57.08 & 94.07 & 24,319 & 89.84 \\
%          \hspace{0.1cm} - AV1 DS* & 57 & 0.11 & 0.18 & 51 & 0.19 \\

%         RTCP & 6,126 & 11.62 & 19.14 & 408 & 1.51 \\
%          - Sender Rep. & 597 & 1.13 & 1.87 & 53 & 0.19 \\
%          - Receiver Rep.* & 394 & 0.75 & 1.23 & 25 & 0.09 \\ 
%          - Transport-CC & 5,135 & 9.74 & 16.05 & 329 & 1.22 \\
        
%          STUN* & 504 & 0.96 & 1.58 & 57 & 0.21 \\
%         \hline
%         Control Plane & 955 & 1.81 & 2.98 & 133 & 0.49 \\
%         Data Plane & 51,777 & 98.19 & 164.79 & 26,937 & 99.51 \\
%         \hline
%         Total & 52,732 & 100 & 164.79 & 27,070 & 100 \\
%     \end{tabular}
%     \vspace{0.1cm}
%     \caption{Packet Types in 5:20 min. WebRTC session.}
%     \label{tab:pkt-types}
% \end{table}

% (1) SFU traditionally have monolithic architecture.
% (2) Majority of work relatively simple, some work fairly complicated (signaling, congestion control, etc.).
% (3) Discuss analogy to SDN: network control (e.g., routing) complex, data plane based on rules from control plane simple (refer back to prev. subsection (dropping, replication)).
% (4) Present overview of split (Figure~\ref{fig:arch}).

While we so far primarily focused on the packet-processing, data-plane aspects of video conferencing, we acknowledge that there are several parts in this workload that require more involved processing, typically more amenable to traditional software running on general-purpose CPUs.
On top of that, controlling the data plane and the rate adaptation logic requires a control plane that is able to process the signaling and the feedback from the media streams.
As a result, we require a decoupled architecture that performs as much as possible in a fast and efficient data plane and runs only tasks that require so in a slower but more programmable, software-based control plane.
Today's monolithic architecture of SFUs~\cite{mediasoup,lopez:kurento,jitsi-videobridge} is not easily amenable to such a split and disaggregating this complex functionality is one of the main challenges we overcome in this work.

% As our analysis of several SFU systems reveals in Section~\ref{}, similar to many networking tasks, the majority of the work in terms of packets to be processed is relatively simple and can be performed in a fast and efficient data plane.
While many tasks a SFU performs naturally map to networking devices as explained in Section~\ref{ssec:arch:sfu-pkt-proc}, SFUs also perform more complex tasks such as signaling, participant management, and congestion control~\cite{webrtc-arch-basics-blog}.
With the exception of congestion control, these tasks run infrequently, e.g, only when a new participant joins or leaves a meeting.
This difference in tasks and their relative frequency is similar to many networking applications, such as routing and has been leveraged for decades in router design and provided the inspiration for SDN~\cite{feamster:road-to-sdn}.

We leverage this insight as well and propose splitting the SFU's functionality into a fast and efficient data plane that can run on efficient (hardware-based) line-rate devices and a slower control plane in software, as shown in Figure~\ref{fig:arch}.
At a high level, the control plane is responsible for signaling, connection establishment, configuring the data plane, and performing congestion control, while the data plane is responsible for media forwarding and performing the actual rate adaptation.
In this architecture, media packets never have to leave the data plane and can be processed entirely in line-rate devices.
In general, except for a small set of packets for initial connection-establishment purposes, no blocking operations are performed in software, overall lowering end-to-end latency of the system.
We will now discuss the exact split between control and data plane and give insight into the different tasks and types of packets processed in each plane.

\noindent
\textbf{Data Plane.}~%
%
% (1) Reiterate involved protocols (refer back to section 2).
% (2) RTP for media, mostly forwarding based on type of packet, RTP can be parsed easily, RTP extensions can also be handled in data plane (under some assumptions, e.g., know identifiers).
% (3) RTCP, mention two different types: SR, RR, TWCC.
% (4) Explain test trace, how was obtained (Table~\ref{tab:pkt-types}).
% (5) Conclude that 98\% of packets, 99.5\% of bytes can stay in data plane.
%
In \S\ref{ssec:background}, we provided a brief overview of the protocols involved in WebRTC and video-conferencing systems in general.
The key protocol here is the Real-Time Transport Protocol (RTP) which is used to transmit media streams.
RTP uses a fixed-sized base header and a variable number of extension headers to carry additional information about the media stream~\cite{rtp-rfc} which makes it amenable to match-action processing in the data plane.
The RTP header is followed by the actual media payload which is typically encrypted while the header is not.

To get a better understanding of the types of packets and the amount of data that is processed in a typical video-conferencing session, we collected a packet-level trace of a unidirectional P2P WebRTC session sending an AV1 video stream using SVC with two temporal layers and an Opus audio stream from one client to another.
We use a basic, self-written WebRTC application written in JavaScript and running in a standard, unmodified Chrome browser.
We then analyzed the trace to determine the number of packets and bytes that can be processed in the data plane and the control plane, respectively.
The results of this analysis are summarized in Table~\ref{tab:pkt-types}.

The experiment ran for 5:20 minutes during which we collected a total of 52,732 packets.
We found that 87.43\% of these packets were RTP packets which can be handled in the data plane with the exception of RTP packets containing an extended AV1 dependency descriptor which however only accounted for 0.11\% of all packets and 0.19\% of all bytes.
We will further elaborate on this packet type in the following section.
RTCP is RTP's control protocol and accounted for 11.62\% of all packets and 1.51\% of all bytes.
RTCP packets are used to convey control information about the media stream and are used for congestion control, reporting, and feedback.
SFUs only use a basic form of congestion control since their capability of adapting the media stream are limited by the use of the respective scalability technology (SVC or Simulcast).
As a result, the input for our SFU-based congestion controller is limited to the RTCP receiver reports (RR) which account for 0.75\% of all packets and 0.09\% of all bytes.
The remaining RTCP packets are sender reports (SR) and transport-cc (TWCC) packets which we forward to the clients and thus can remain entirely in the data plane.
In the future, a hybrid model where RTCP Transport-CC messages are processed in the control plane when the receiver reports indicate congestion might be beneficial.

In summary, 98.19\% of all packets and 99.51\% of all bytes can be processed in the data plane, making this workload naturally suited for such a control/data-plane split.
Almost more importantly, the remaining packets with the exception of a few STUN packets at the beginning of each session are not blocking.

\noindent
\textbf{Control Plane.}~%
% (1) Mention signaling, say not included in this table, say when and how many messages.
% (2) Dependency structure, why cannot be in data plane.
% (3) Receiver report, what contains, needs to be in controller not because of complexity of message but rather because that's where next rate is computed. Comment that it might be possible to detect anomalies and if everything is perfect, no need to forward to control plane.
% (4) TWCC, mention that not useful for coarse-grained adaptation at SFU but used at client, so should be forwarded there.
% (5) STUN, say that requires HMAC, could potentially be done in accelerator.
% (6) no actions except for initial STUN are synchronous, acknowledge need for timely feedback of RTCP RRs.
%
The control plane is responsible for all tasks not amenable to efficient data-plane processing.
This can be either due to (1) the complexity of the task or (2) the complexity of the header format of the relevant packets to be processed.
We find that with the exception of performing congestion control, the reason for control-plane processing is rather due to the complexity of the header format.
We will discuss possible changes to the involved protocols to make them more amenable to data-plane processing in \S\ref{sec:discussion}.

The key tasks of the control plane are to (1) perform congestion control, (2) handle signaling and connection establishment, and (3) extract information from the media stream that are relevant for rate adaptation.
First, our congestion control interface is based on RTP receiver reports, these reports are sent periodically by a stream receiver and contain information about the quality of the received media stream, in particular the receive jitter and fraction of packets lost.
These metrics are then used to select the appropriate downstream configuration (i.e., the set of scalability layers to forward) for a given participant.

Second, the control plane is responsible for signaling and connection establishment.
Signaling refers to the process of exchanging capabilities and connection-related information between peers.
This is typically done using the Session Description Protocol (SDP)~\cite{sdp-rfc} which is carried out-of-band often over a Websocket or another type of separate TCP connection and is as such not a  function of an SFU even though some SFUs perform this task.
Our prototype is also bundled with a signaling server that is responsible for this task.
The signaling messages are only exchanged when a new participant joins or leaves a meeting and are thus very infrequent and can be handled by the software-based control plane or an external signaling server.
Connection establishment and maintenance is typically performed using the STUN protocol~\cite{stun-rfc} which is used to discover the presence of network address translators (NATs) and firewalls between peers.
STUN messages are sent over UDP, have a relatively complex, variable-length header format and require the computation of a HMAC which typically requires software involvement.
Our trace contained 504 STUN packets (0.96\% of all packets) and 57 Kilobytes (0.21\% of all bytes) and are thus comparatively infrequent and can be handled by the control plane.

Finally, the control plane is responsible for extracting information from the media stream that is relevant for matching the correct SVC meta data for rate-adaptation purposes.
The AV1 codec, for example, uses a dependency descriptor that is transmitted every time the structure of the SVC stream changes.
The layer identifiers included in this descriptor can then later be used to selective forward specific layers.
While this dependency descriptor is difficult to parse and requires software processing, it only appears infrequently, and mostly at the beginning of a stream while the available bandwidth is still being probed.
Our trace contained 57 such packets, or 0.11\% of all RTP packets.

\subsection{Introducing \sys}
\label{ssec:intro-p4-sfu}

Based on the insights we gained from our analysis which demonstrate an opportunity for a more-efficient, disaggregated architecture for Selective Forwarding Units, in this paper, we propose a novel architecture and prototype system, which we call \sys.
As the foundation of our system, we leverage the WebRTC standard~\cite{w3c:webrtc}.
WebRTC is an open-source standard and protocol specification that enables real-time communication over the Internet.
WebRTC can be used from browsers where it is implemented and available through a JavaScript API in all major browsers or by using \texttt{libwebrtc}, a C++ library that provides the same functionality but is significantly harder to use.
WebRTC is used (sometimes with some modifications) in several major video-conferencing systems, such as Microsoft Teams~\cite{ms-teams} and Google Meet~\cite{google-meet}.

The data plane of our \sys{} prototype is based on the P4 language and the PISA architecture and is designed for an Intel Tofino switch~\cite{intel:tofino}.
The Tofino is a 3.2 Tbit/s+ fully-programmable switch ASIC designed for data centers and enterprise networks.
Our design, however, is not specific to this device and our division of labor as well as our P4-based implementation can easily be modified for SmartNICs, FPGAs, or other programmable data-plane devices.

==> sec/archive/arch2.tex <==
\section{Design Overview}

The packet-level operation of an SFU exposes striking similarity with key networking tasks that are commonly implemented in high-performance network devices in order to scale to high data rates.
Based on this insight which demonstrates an opportunity for a more-efficient, disaggregated architecture for Selective Forwarding Units, in this paper, we propose a novel architecture and prototype system, which we call \sys.
As the foundation of our system, we leverage the WebRTC standard~\cite{w3c:webrtc}.
WebRTC is an open-source standard and protocol specification that enables real-time communication over the Internet.
It can be used in all major browsers where it is implemented and available through a JavaScript API or by using \texttt{libwebrtc}, a C++ library that provides the same functionality but is significantly harder to use.
WebRTC is used (sometimes with modifications) in several major video-conferencing systems, such as Microsoft Teams~\cite{ms-teams} and Google Meet~\cite{google-meet}.

% In the previous section we have shown how the core functionality of an SFU can operate primarily on a packet level by forwarding replicas of media packets and selectively dropping packets in order to reduce the outgoing media bitrate to accommodate for receiver capabilities or network capacity.
% Forwarding packets along a tree-like topology is akin to multicast routing while selectively dropping packets is the key functionality of packet filters.
% Consequently, the packet-level operation of an SFU exposes striking similarity with key networking tasks that are commonly implemented in high-performance network devices in order to scale to high data rates.
% Based on this insight, in this paper, we explore how to treat video conferencing as a packet-processing workload which then enables offloading data-plane functionality to efficient hardware devices and accelerators.
% We do so by proposing a new architecture for video-conferencing systems and presenting Scallop, a novel hardware/software co-designed SFU that implements this architecture.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{fig/arch.pdf}
    \caption{Scallop Architecture.}
    \label{fig:arch}
    % \vspace{-0.3cm}
\end{figure}

While we so far primarily focused on the packet-processing, data-plane aspects of video conferencing, we acknowledge that there are several parts in this workload that require more involved processing, typically more amenable to traditional software running on general-purpose CPUs.
On top of that, controlling the data plane and the rate adaptation logic requires a control plane that is able to process the signaling and the feedback from the media streams.
As a result, we require a decoupled architecture that performs as much as possible in a fast and efficient data plane and runs only tasks that require so in a slower but more programmable, software-based control plane.
Today's monolithic architecture of SFUs~\cite{mediasoup,lopez:kurento,jitsi-videobridge} is not easily amenable to such a split and disaggregating this complex functionality is one of the main challenges we overcome in this work.

% As our analysis of several SFU systems reveals in Section~\ref{}, similar to many networking tasks, the majority of the work in terms of packets to be processed is relatively simple and can be performed in a fast and efficient data plane.
While many tasks an SFU performs naturally map to networking devices, SFUs also perform more complex tasks such as signaling, participant management, and congestion control~\cite{webrtc-arch-basics-blog}.
With the exception of congestion control, these tasks run infrequently, e.g, only when a new participant joins or leaves a meeting.
This difference in tasks and their relative frequency is similar to many networking applications, such as routing and has been leveraged for decades in router design and provided the inspiration for SDN~\cite{feamster:road-to-sdn}.

We leverage this insight as well and propose splitting the SFU's functionality into a fast and efficient data plane that can run on efficient (hardware-based) line-rate devices and a slower control plane in software, as shown in Figure~\ref{fig:arch}.
At a high level, the control plane is responsible for signaling, connection establishment, configuring the data plane, and performing congestion control, while the data plane is responsible for media forwarding and performing the actual rate adaptation.
In this architecture, media packets never have to leave the data plane and can be processed entirely in line-rate devices.
In general, except for a small set of packets for initial connection-establishment purposes, no blocking operations are performed in software, overall lowering end-to-end latency of the system.
We will now discuss the exact split between control and data plane and give insight into the different tasks and types of packets processed in each plane.

==> sec/archive/background.tex <==
% !TEX root = ../p4-sfu-nsdi24.tex  

\section{Background}
\label{sec:background}

\textcolor{blue}{
Before elaborating in more detail on Selective Forwarding Units (SFU), in this section we provide a brief overview of the components and tasks involved in establishing and maintaining a video conference and the different architectures that are used to interconnect meeting participants.
}
Video-conferencing applications (VCAs) are complex distributed systems with many different protocols and components that need to work in concert.
\textcolor{blue}{
In a nutshell, the three principal functions that a VCA must perform are: (1) negotiating client capabilities and establishing a connection between participants (signaling), (2) exchange media streams between participants (media forwarding), and (3) adapting media streams to the network conditions, device capabilities, or preferences of individual participants (rate adaptation), which we will now describe in more detail.
}

% For example, typical protocols include RTP and RTCP for media transmission, SIP and SDP for signaling, and STUN for connection establishment.
% More background on VCAs and these protocols can be found in~\cite{nistico:comparative-study-rtc, blum:webrtc, rtp-rfc, rtp-av-conference-rfc, sdp-rfc, srtp-rfc, ice-rfc, schwarz:svc-overview, lee:demystifying-vca}.
% For this paper, we now provide background on the ways meeting participants can be interconnected and how media is forwarded between them.



\textbf{Signaling.}

\textbf{Media Forwarding.}

\textbf{Rate Adaptation.}



\textbf{Peer-to-Peer Meetings.}
Direct peer-to-peer (P2P) connections between meeting participants result in the lowest latency between two given clients but can be challenging to realize in the presence of firewalls and network address translators (NAT)~\cite{ice-rfc,baset:analysis-of-skype,ford:p2p-across-nat}.
The left side of Figure~\ref{fig:call-arch} depicts the media streams in a three-party P2P meeting.
Large P2P meetings put significant load on each sender as different versions of the media must be encoded to match different receiving participant's device and network capabilities (as illustrated by the dashed lines).
Moreover, as each sender sends an individual media stream per other participant, this approach requires substantial uplink bandwidth which is often not available in residential and wireless Internet access settings.
As a result, most VCAs use P2P connections only for some two-party calls (e.g., Zoom) or not at all (e.g., Google Meet)~\cite{nistico:comparative-study-rtc, michel:passive-measurement-zoom, lee:demystifying-vca}.

\textbf{Intermediate Servers.}
To avoid the uplink bottleneck problem, intermediate servers were introduced that either transcode incoming streams to a single outgoing stream per participant or one that selectively replicates and forwards media streams among clients.
The server in the latter case is called a Selective Forwarding Unit (SFU) which is the de-facto standard in video conferencing today.
Similar intermediate servers are used for live-streaming use cases.
The topology in terms of media streams of a three-party SFU-based meeting is depicted on the right side of Figure~\ref{fig:call-arch}.
A SFU receives each client's media streams, replicates the streams for each downlink participant and forwards the media accordingly.
This approach reduces the amount of uplink bandwidth required at the clients but, depending on the location of the SFU relative to the meeting participants, may significantly increase delay.

\textbf{Heterogenous Participants and Rate Adaptation.}
As previously mentioned, a SFU must adapt media streams for the network conditions, device capabilities, or preferences of individual downstream meeting participants.
To enable this functionality, the SFU receives a high-quality source stream from each participant and then \emph{selectively} forwards subsets of this stream to the other participants; this is possible through Simulcast~\cite{lin:gso-simulcast} or Scalable Video Coding (SVC)~\cite{w3c:webrtc-svc, schwarz:svc-overview}.
In SVC, a scalable video stream contains several layers corresponding to different quality levels where higher-quality layers build upon lower-quality layers.
The SFU can then remove higher-quality parts of a video bit stream to adjust video resolution, frame rate, or picture quality, ultimately reducing the data rate to send to a participant.
Of course, the SFU must also decide what the most appropriate sending rate for a participant is through a rate controller that receives periodic reports from receivers containing loss and jitter information.
% Other signals for rate-adaptation purposes are available including \emph{transport-wide congestion control}~\cite{carlucci:google-cc} and NACKs.


==> sec/archive/conclusion.tex <==
% !TEX root = ../p4-sfu-nsdi24.tex  

\section{Conclusion}
\label{sec:conclusion}

This paper presents the design and implementation of \sys{}, a bold rearchitecting of video-conferencing infrastructure to tackle scalability challenges as video-conferencing traffic increases. Our SDN-inspired SFU-switch design is driven by the key insight that most SFU tasks are, in fact, replicating and dropping media packets. Unlike traditional infrastructure where an SFU server takes care of everything, our \sys{} prototype comprises an efficient programmable data plane that processes media packets at line rate and a software control plane that handles infrequent tasks such as signaling, connection setup, quality monitoring, and congestion control. Our prototype is built with a commodity server and a real programmable switch (Intel Tofino~\cite{intel:tofino}). It works with an existing real-time multimedia protocol, WebRTC, with participating clients using unmodified Chrome web browsers. Our analysis and evaluation with Zoom traffic captured at a production campus network show that \sys{} delivers 20-40x improved scalability over a 32-core SFU server. 
%Our Tofino-based implementation
%fully supports WebRTC, and delivers 20-40× improved scal-
%ing over a 32-core commodity server, while reaping perfor-
%mance improvements by avoiding contention-induced jitter.
%Fueled by this insight, we present \textbf{\sys{}}, an SDN-inspired WebRTC SFU design and system that decouples VCA infrastructure into (1) an efficient data plane that relays media packets using line-rate network switching hardware, and (2) a software control plane that handles the remaining, \emph{infrequent} tasks (e.g., signaling, quality monitoring, congestion control, and connection setup). Realizing this vision with existing real-time multimedia protocols and constrained line-rate network devices poses numerous challenges, described in turn.
% \

==> sec/archive/control.tex <==
% !TEX root = ../p4-sfu-nsdi24.tex  

\section{Control-Plane Implementation}
\label{sec:control}

The control plane is responsible for all tasks not amenable to efficient data-plane processing.
This can be either due to (1) the complexity of the task or (2) the complexity of the header formats of the relevant packets.
We find that, with the exception of performing congestion control, the reason for control-plane processing is most commonly due to the complexity of the header format.
We will discuss possible changes to the involved protocols to make them more amenable to data-plane processing in \S\ref{sec:discussion}.
The key tasks of the control plane are to (1) perform congestion control, (2) handle signaling and connection establishment, and (3) extract information from the media stream that is relevant for rate adaptation.

% \noindent
\subsection{Hierarchy of Control Software}

While all the before-mentioned tasks require processing capabilities that exceed those of a hardware switch, they can be further subdivided in such tasks that potentially require a global view of the system if SFUs form a hierarchy (so called cascading SFUs) and those that are local to one forwarding device (a switch in our case).
The second distinction are those tasks that are potentially latency-sensitive and those that only happen infrequently during a time where changes to the call are applied (e.g., participants joining and leaving).
Luckily, the tasks that require a global view are also those that are not latency-sensitive and vice versa.

Consequently, our system is built using a two-layer control plane where a software component handles---directly on the switch CPU---all the tasks that the switch cannot perform and can potentially be latency sensitive. This minimizes the latency between the controller and the switch to the sub-millisecond range.
% \jrex{sentence is hard to parse}.
This architecture is depicted in Figure~\ref{fig:control}.
This part of the controller that we call \emph{Switch Agent} is directly connected to the switch data plane via an internal port and is more akin to a side car to the switch.
All remaining tasks are those that require a global view and are implemented in a centralized controller.
This controller is comparable to a traditional network controller as found in SDN deployments.
While we have not implemented cascading SFUs in our prototype, this split that our implementation leverages directly enables this functionality.
We will now describe the two components of the control plane in detail.

% \noindent
\subsection{Central Controller}

The key function of the central controller is signaling and distributing forwarding rules to the switch, which are derived from its bird's-eye view of all meetings, their participants, and shared media streams that the system is handling at any given point in time.
The controller maintains this view and state about all meetings since it is also the system's signaling server.
Signaling is the process of exchanging capabilities and connection-related information between peers.
We implement this using the Session Description Protocol (SDP)~\cite{sdp-rfc} which is carried over a Websocket connection.
Signaling messages are only exchanged when a new participant joins or leaves a meeting and are thus very infrequent and can be handled by the software control plane or an external signaling server.
Scallop relies on controlling the signaling messages as it needs to tell the clients where to send traffic (i.e., the SFU), what media codecs, and feedback mechanisms to use.








\subsection{Switch Agent}

The switch agent is a lightweight process that runs on the switch CPU (in our case an 8-core Intel Pentium) and has a direct connection to the data plane using a virtual port of the switch.
As a result, it is located between the centralized controller and the data plane and translates messages about new or removed media streams (derived from signaling messages) into data-plane rules to be installed on the switch.
It implements an interface for congestion control by making RTCP feedback signals available to a function where they are analyzed.
Similarly, this function has access to an API that can control the set of quality layers to be forwarded to the participant the feedback signal was received from.
We explain this process in more depth next.

Second, the switch agent handles all STUN communication.
STUN is a protocol to enable traversal of NATs.
While \sys{} needs to run bound to an IP address that is reachable from each client, the clients are commonly behind a firewall and NAT (especially in residential settings).
STUN enables the controller (and thus the SFU) to determine the Internet-facing IP address of the client.
Additionally, STUN is used for periodic connectivity checks between clients and the SFU.
The required STUN messages are sent over UDP, have a relatively complex, variable-length header format, and require the computation of an HMAC which typically requires software involvement.
Our data plane sends all packets to the switch agent where responses to initial NAT traversal, connection establishment, and connectivity check packets are generated and passed back through the data-plane/switch-agent port.
In a representative trace trace collected from \sys{}, STUN accounts for 0.35\% of all packets and is thus comparatively infrequent and can be handled by the control plane (see \S\ref{subsec:control-eval} for details).

Finally, the control plane is responsible for extracting information from the media stream that is relevant for matching the correct SVC meta data for rate-adaptation purposes.
We use the AV1 video codec and its dependency descriptor that is transmitted every time the structure of the SVC stream changes~\cite{av1}.
The layer identifiers included in this descriptor need to be processed and stored at the switch agent to then later enable selective forward of specific layers.
There is a strict association between a specific quality configuration of the stream and the set of layer identifiers that need to be dropped or forwarded to use the respective quality configuration.
While this dependency descriptor is difficult to parse and requires software processing, it only appears infrequently whenever the encoder resolution changes or a key frame is generated which in this workload only happens if (a) a new participant joins, (b) a picture is entirely lost and the decoding chain has been broken in a way that retransmissions cannot repair the decoder state, or (c) the resolution at the encoder changes.
Otherwise, video-conferencing traffic uses a sequence of P-frames for inter-frame prediction.

It is important to note that none of these operations, except for the very first set of STUN packets that are used for initial connection establishment and NAT traversal are blocking in the sense that their (software-based) processing would have to conclude before a media packet can be forwarded. This is because only copies of those packets are sent to the switch agent while the packets are already being forwarded in the data plane.
As a result, packets going to the switch agent do not have an impact on the performance of the session (e.g., relating to QoE).

% First, our congestion control interface is based on RTP receiver reports, these reports are sent periodically by a stream receiver and contain information about the quality of the received media stream, in particular the receive jitter and fraction of packets lost.
% These metrics are then used to select the appropriate downstream configuration (i.e., the set of scalability layers to forward) for a given participant.

% Second, the control plane is responsible for signaling and connection establishment.
% % Signaling refers to the process of exchanging capabilities and connection-related information between peers.
% This is typically done using the Session Description Protocol (SDP)~\cite{sdp-rfc} which is carried out-of-band often over a Websocket or another type of separate TCP connection and is as such not a  function of an SFU even though some SFUs perform this task.
% Our prototype is also bundled with a signaling server that is responsible for this task.
% The signaling messages are only exchanged when a new participant joins or leaves a meeting and are thus very infrequent and can be handled by the software-based control plane or an external signaling server.
% Connection establishment and maintenance is typically performed using the STUN protocol~\cite{stun-rfc} which is used to discover the presence of network address translators (NATs) and firewalls between peers.
% STUN messages are sent over UDP, have a relatively complex, variable-length header format and require the computation of a HMAC which typically requires software involvement.
% In our trace, STUN accounts for 0.35\% of all packets and is thus comparatively infrequent and can be handled by the control plane.

% Finally, the control plane is responsible for extracting information from the media stream that is relevant for matching the correct SVC meta data for rate-adaptation purposes.
% The AV1 codec, for example, uses a dependency descriptor that is transmitted every time the structure of the SVC stream changes.
% The layer identifiers included in this descriptor can then later be used to selective forward specific layers.
% While this dependency descriptor is difficult to parse and requires software processing, it only appears infrequently, and mostly at the beginning of a stream while the available bandwidth is still being probed.
% Our trace contained 57 such packets, or 0.11\% of all RTP packets.

% \textbf{}



% \noindent
% \textbf{Central Controller.}~%
% Describe session management, esp. Multiple peer connections per participant for CC purposes (diagram with signals / associated control loops) and SDP signaling

% \noindent
% \textbf{Switch Agent.}~%
% \begin{itemize}
%     \item STUN needs to be handled in software control plane due to HMAC computation
%     \item Congestion control uses RTCP receiver reports + REMB
%     \item Analyzes AV extended dependency descriptors to associate quality layers with layer id’s from media stream
%     \item None of the operations are blocking within the media stream except for initial STUN connection establishment
%     \item If WebRTC was more hardware-amenable and if the switch would support more basic message authentication / crypto operations, the role of the switch agent becomes less and less important
% \end{itemize}

\subsection{Feedback Handling}

% \begin{figure}[t]
%     % \centering
%     \centering
%     \begin{minipage}[t]{0.49\textwidth}
%         \includegraphics[width=\columnwidth]{fig/control.pdf}
%         \caption{\sys{} Control Plane Messages}
%         \label{fig:control}
%     \end{minipage}
%     \hspace{0.4cm}
%     \begin{minipage}[t]{0.45\textwidth}
%         \includegraphics[width=\columnwidth]{fig/rtcp-fwd.pdf}
%         \caption{RTCP Report Forwarding and Aggregation}
%         \label{fig:rtcp-fwd}
%     \end{minipage}
% \end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{fig/control.pdf} % for 2-column layout
    % \includegraphics[width=0.35\columnwidth]{fig/peer-conn.pdf} % for 1-column layout
    \caption{Use of WebRTC PeerConnection API}
    \label{fig:peer-conn}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{fig/rtcp-fwd.pdf} % for 2-column layout
    % \includegraphics[width=0.45\columnwidth]{fig/rtcp-fwd.pdf} % for 1-column layout
    \caption{RTCP Report Forwarding and Aggregation}
    \label{fig:rtcp-fwd}
\end{figure}

\noindent
\textbf{Feedback Messages.}
RTP uses its sister protocol, RTCP, the Real-Time Transport Control Protocol to provide feedback signals about the receive quality of a stream to the sender.
The sender then uses these messages for congestion-control purposes.
WebRTC uses the Google Congestion Control (GCC)~\cite{carlucci:google-cc} algorithm that can run in two different modes.
The first mode is sender-driven where per-packet one-way delay gradients are reported by the receiver and sent to the sender inside a \emph{transport-cc} message where the bandwidth estimate is then computed.
In the second mode, the receiver-driven mode, the receiver directly computes the estimated bandwidth based on the packet arrival time variation and sends the result of this computation inside a \emph{Receiver-estimated bandwidth (REMB)} message back to the sender where the encoder is instructed to match this capacity.
\sys{} uses receiver-driven congestion control as maintaining transparency with sender-driven CC would require us to rewrite sequence numbers inside the feedback messages when quality layers are dropped.
This format is too complex for the data plane and would put significant load on the switch agent as in this case the packets would also have to be forwarded from software, making the operation blocking.
Additionally, using REMB messages has the advantage that \sys{} can directly leverage the estimated bandwidth inside the data plane to perform rate adaptation on the respective media stream in case of congestion and does not have to compute an estimate itself.

\noindent
\textbf{Forwarding of RTCP Messages.}
\sys{} handles RTCP receiver reports (RRs) providing coarse-grained loss and jitter information, RTCP sender reports (SRs) providing statistics about a sent stream to receivers, negative acknowledgments (NACKs) reporting lost packets, picture-loss indications (PLIs) reporting a broken decoding chain, and finally REMB messages providing the aforementioned bandwidth estimate.
The way \sys{} processes and forwards these messages is depicted in Figure~\ref{fig:rtcp-fwd}.
Sender Reports are replicated and forwarded from senders to all receivers of the particular stream.
This uses the same logic as forwarding media packets within the data plane.
RRs and REMB messages are forwarded in the data plane such that only the reports of the currently best-performing receiver are being forwarded to the respective sender.
We determine this receiver by computing a moving average over the bandwidth estimates for each individual receiver and then periodically comparing the current moving average value across all the receivers of the stream. The receiver reports and REMB messages of the participant whose smoothed estimated bandwidth is the maximum of all receivers get forwarded to the sender.
The rationale behind this is that the sender should encode the maximum possible quality and let the SFU take care of selectively reducing the rate for individual receivers with poor-performing connections.
If a random receiver report would be chosen to forward to the sender, all receivers would be penalized by receiving a potentially lower-quality stream tailored to the participant that sent the report.
Finally, PLIs and NACKs originate at a single receiver and are forwarded to the respective sender.

\noindent
\textbf{Use of Multiple Peer Connections per Participant.}
Finally, opposite to typical use of WebRTC where all media streams are multiplexed over a single \emph{RTCPeerConnection} which effectively corresponds to a UDP flow, in \sys, each participant uses a dedicated peer connection to send media and a dedicated peer connection for each other participant in the meeting. This setup is depicted in Figure~\ref{fig:peer-conn}. The controller manages the setup and maintains the correct associations of these connections and flows and configures the data plane accordingly. The reason for this design choice is that otherwise, the use of combined RTCP REMB messages (one packet to report about multiple received streams) would require splitting the messages in the data plane in order to only forward the messages relevant to a particular sender to the sender.
Furthermore, combined peer connections result in feedback signals that incorporate all links within the meeting topology and, as a result, are not useful for rate adaptation as they are not specific to one sender-receiver pair.
Since the feedback signal operates on peer connections rather than media connections, using a dedicated peer connection per media stream keeps feedback specific to one stream which is the granularity that the sender and SFU use to adapt the quality.



% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=0.85\columnwidth]{fig/peer-conn.pdf} % for 2-column layout
%     \includegraphics[width=0.45\columnwidth]{fig/peer-conn.pdf}
%     \caption{Use of WebRTC PeerConnection API}
%     \label{fig:peer-conn}
% \end{figure}


% % Consider Problem 1 in Figure~\ref{rtcp-problem}, the REMB packets sent from participant 3 include two with information about the bandwidth  
% Secondly, as a result of our proxy (as opposed to split proxy) design, the REMB messages also include information about the path between the sender and the SFU.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.99\columnwidth]{fig/rtcp-problem.pdf}
%     \caption{Issues associated with combined peer connections.}
%     \label{fig:rtcp-problem}
% \end{figure}



% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.99\columnwidth]{fig/rtcp-solution.pdf}
%     \caption{Use of WebRTC PeerConnection API}
%     \label{fig:peer-conn}
% \end{figure}


==> sec/archive/data.tex <==
% !TEX root = ../p4-sfu-nsdi24.tex  

\section{Data-Plane Implementation}
\label{sec:data}

The data-plane operation of the SFU can be subdivided into three concrete sub-tasks, all of which primarily aim to bridge the gap between network-layer packet processing and application-layer semantics. 
In this section, we describe these sub-tasks, and explain our solution approach to each of them.
Since we implemented and deployed our system on the Intel Tofino high-speed programmable switch, some of the specifics of the data-plane implementation go into details about the programmable constructs offered by the Tofino, and their advantages and limitations. However, we posit that these constructs are not just limited to the Tofino, but are broadly available on other programmable packet-processing hardware as well, such as SmartNICs and FPGAs. Therefore, our techniques are more general than being restricted to our platform of choice. On the contrary, the fact that we can implement our solution on the Tofino, which comes with one of the most restrictive sets of compute and memory constraints among packet-processing hardware (to extract high performance), provides us confidence that our solution can be implemented on other programmable packet processors as well.

% One key insight of our paper is that the operation of a video-conferencing SFU is strikingly similar to packet processing.
% However, packet processing, which can include packet replication and dropping (for rate adaptation), requires application context.
% For example, a video packet of an SVC enhancement layer could be subject to both replication and rate adaptation, a video packet of an SVC base layer or an audio packet to only replication, a feedback packet to either replication (e.g., a sender report) or selective forwarding (e.g., a receiver report). \joon{I cannot actually understand this last sentence.}

\subsection{Flexible Recursive Parsing}
\label{subsec:parsing}

%Understanding the context in which a packet appears requires parsing deep into the packet headers, right down to the application layer.
%In WebRTC, different extension header types can follow the base application-layer header (i.e., RTP/RTCP). One packet can have multiple of these extensions, often in variable length, stacked on top of each other and interspersed with padding. This renders deep parsing non-trivial, requiring multiple recursive parsers (one for each extension type) to operate simultaneously with the flexibility to accommodate skip-overs (for padding).
%Unfortunately, the header parser of a high-speed programmable switch (e.g., the Intel Tofino) is equipped with limited recursive parsing capabilities (e.g., one \texttt{ParserCounter}), forcing us to develop our own flexible recursive parsing scheme.
%Our key insight is that a recursive parser can be constructed by unrolling it into a list of identical parser states, with each parser state tagged with the byte position of the packet where the state was encountered (e.g., $S_0$, $S_1$, ..., $S_{16}$). We write a program to auto-generate this list of states, given a maximum byte position, which we set to the maximum byte position in a packet where we have encountered this state in our WebRTC traces. At each state (say, $S_n$), we read the length of the extension (say, $m$), and jump to the corresponding lower state ($S_{n-m}$), until we reach $S_0$. We also accommodate padding, by including the option to skip over it in each listed state.

To understand the semantic context in which a packet appears, we need to parse deep into the packet headers, right down to the application layer. However, 
in WebRTC, the base application-layer header (i.e., RTP/RTCP) can be followed by different extension header types. Furthermore, each packet can have one or more of these extensions stacked on top of each other. Sometimes, these extensions are even interspersed with padding. While it is trivial for a software-based packet parser to parse these dynamic headers, since we implement our data plane in a resource-constrained hardware switch, we do not readily have the same ability. Instead, we build our own flexible and recursive parser using the parsing capabilities offered by the switch. Our construction involves "unrolling" the recursive parser into a list of states with identical functionality, but with different names, where the state name also reflects the current recursion depth (e.g., \texttt{state parse\_onebytehdrtype\_depth1}). We also accommodate padding in a similar way, and maintain a separate recursion tree for it.
While previous work has implemented deep parsers on the Tofino to support stacked dynamic-length headers, this way of interleaving two parser recursion trees is novel. \oliver{Citation?}

% multiple of these extensions stacked on top of each other and interspersed with padding. This renders deep parsing non-trivial, requiring multiple recursive parsers (one for each extension type) that also accommodate skip-overs (for padding).
% Unfortunately, the header parser of a high-speed programmable switch has limited recursive parsing capabilities.
% We construct this parser by unrolling it into a list of identical parser states, with the name of the state also including the current recursion depth.

% with each state tagged with the byte position of the packet where the state was encountered (e.g., $S_0$, $S_1$, ..., $S_{16}$). We write a program to auto-generate this list of states, given a maximum byte position, which we set to the maximum byte position in a packet where we have encountered this state in our WebRTC traces. At each state (say, $S_n$), we read the length of the extension (say, $m$), and jump to the corresponding lower state ($S_{n-m}$), until we reach $S_0$. We also accommodate padding, by including the option to skip over it in each listed state.

% We believe other applications that require deep and flexible header parsing capabilities can leverage such a strategy in the future. 
% \joon{yeah, this is hard to understand. Not sure if it's worth trying to explain, actually. Do you think the technique is unique and interesting enough to make P4 developers like it?}

\subsection{Replication and Selective Forwarding}
\label{subsec:replication}

% Understanding a packet’s context via deep parsing only helps determine the action that needs to be taken on the packet. Implementing the actual action may come with additional challenges.

Our parser enables us to gain visibility into the semantic context of each packet, which then allows us to decide the appropriate set of actions to apply to it. However, performing these actions may come with additional challenges.
For instance, if the context demands replication, traditional multicasting does not suffice since multiple receivers may be downstream of the same egress port and not all receivers always receive all packets (i.e., during rate adaptation). Fortunately, the data plane's packet replication engine (PRE) offers an opportunity to create multiple packet replicas per egress port.
The PRE allows the construction of a three-level replication tree; the first level (i.e., the root) is identified by a multicast group ID, the second level by a replication node ID, and the third (i.e., the leaf) by a physical egress port. 
Multiple second-level nodes can have the same third-level nodes, which allows sending multiple packet replicas to the same egress port.
% Since multiple second-level nodes can have the same third-level nodes, sending multiple packet replicas to the same egress port is possible.

However, it is not obvious what the nodes at each level of the PRE should represent in the context of a WebRTC meeting. For example, a node could represent a group of meetings, one unique meeting, a unique participant, a unique media stream, and so on. Also, the number of nodes at each level is limited by the size of the tables that are used to administer the PRE, meaning we will quickly run out of PRE resources if we construct too many replication trees per meeting. 
Then again, if we aggregate multiple entities (e.g., meetings) into one tree, then we could end up with far too many replicas, thereby cutting down the effective bandwidth of the egress pipeline and needing it to drop a great many of them. \oliver{last part of previous sentence is awkward.}
We observe that it is possible for the PRE to function correctly if we create one replication tree per sending participant in a meeting. However, this strategy results in quadratic scaling of PRE resource consumption and is therefore not ideal. Rather, we achieve a better balance between PRE resources and egress bandwidth by creating one replication tree per meeting. All streams (media or feedback) within a meeting can then be replicated to all other participants using just a single replication tree. We simply suppress the branch (discussed next) that corresponds to the sender of the stream. We refer to this strategy as the optimized version of the PRE.

Fortunately, the PRE of the Tofino has the provision to suppress certain branches of the replication tree on a per-packet basis. This enables us to go one step further in efficient packet processing -- instead of dropping a media packet that is no longer needed as a result of rate adaptation, we don't even generate it in the first place.
We believe that while our replication solution is specific to our use case, this way of reasoning about the best utilization of the replication capabilities of a packet-processing device can be of benefit to future studies.

% \joon{This is also somewhat hard to follow. But I think this is a pretty important technique, that shines in section 6? If this implementation technique is novel and important enough, it might be worth to use a diagram to explain this. Another question: right now,
% it reads like this is very Tofino-specific. Is this the case? Then reviewers might think, 'bah, not applicable to other targets. not good.' So, if we think this is not Tofino-specific, we should show this somehow.}

\subsection{Transparent Rate Adaptation}
\label{subsec:transparent}

Suppressing (or intentionally dropping) 
% \joon{is suppressing and dropping the same thing here? Best to be consistent} 
certain packet replicas in this way creates an additional challenge. Each packet in a media stream is uniquely identified by a sequence number. When we suppress packets, the receiver observes gaps in sequence numbers, causing it to request retransmissions, which defeats the purpose of suppression. Instead, \sys{} needs to suppress undesired media packets transparently to the receiver. It is important to note that while Zoom also uses an SFU that  suppresses packets to perform rate adaptation, it does not need to rewrite sequence numbers because it has control over the end-host (i.e., via the Zoom client app) and can instrument the client to ignore gaps in sequence numbers caused by suppression by the SFU. This is in sharp contrast with our setting where our client is a generic web browser and we want to remain compliant with WebRTC, which expects a continuous stream of sequence numbers for interrupted operation. Even in cases where a Zoom meeting takes place over a browser (which is deprecated and discouraged by Zoom), they tunnel the traffic over a WebRTC data channel thereby bypassing the standard WebRTC mechanism, which also results in significant performance degradation~\cite{zoom-web-client}.

To handle the gaps in sequence numbers when a media stream has been subject to rate adaptation, we implement a strategy to rewrite sequence numbers. A naive algorithm would store the number of suppressed packets (say, $suppress\_count$) per media stream, and generate the new sequence number as the difference between the original sequence number contained in the packet and this $suppress\_count$.
Unfortunately, this suffers from a crucial flaw. Let's say packets $P_1$, $P_2$ comprise the base layer of the video frame $F_1$, packets $P_3$, $P_4$ comprise the enhancement layer of frame $F_1$, and packets $P_5$, $P_6$ comprise the base layer of the next frame $F_2$. Let's say that $P_1$ had the sequence number $1$, $P_2$ has 2, and so on. The frames belong from a video stream where the enhancement layer should currently be suppressed due to rate adaptation. If $P_1$, $P_2$, and $P_4$ arrive at \sys{} (assuming $P_3$ is lost in the network), it will only add $1$ to $suppress\_count$ due to $P_4$, instead of $2$ due to both $P_3$ and $P_4$. Now, if $P_5$ arrives, its sequence number is computed as its original sequence number (i.e., $5$) minus the $suppress\_count$ (i.e., $1$), which makes the rewritten sequence number $4$, while it should have been $3$. This would be fine, except $P_3$ now arrives (it was reordered in the network), causing the $suppress\_count$ to now (finally) increase to $2$. Now if $P_6$ arrives, notice that the rewritten sequence numbers for both $P_5$ and $P_6$ will now be $4$, thereby confusing the downstream receiver.
% \joon{why? P5 is subject to count 1 and P6 is subject to count 2. Why same?}

To address this and similar issues due to reordering and bursty loss (packets over multiple consecutive frames lost together) in the network upstream of \sys, we design an algorithm that maintains two invariants: (1) the rewritten sequence numbers are always in the same order as the original sequence numbers, and (2) the rewritten sequence numbers never hide an actual loss in the network upstream of \sys. We achieve this by maintaining a small amount of flow state; in addition to the $suppress\_count$, we also store information about the latest frame seen (whether it’s a suppressed frame and whether we have encountered its last packet). Essentially, in the face of loss and reordering, we compute our most conservative estimate of the $suppress\_count$, and never increase it even if reordered suppressed packets appear.
This leaves the potential for extra gaps to appear in the rewritten sequence numbers, but our experiments show that while this leads to some erroneous extra retransmissions, it has a negligible impact on the quality of the call at loss rates observed in our campus network. 
%\oliver{I'm unclear why extra retransmissions have impact on the call quality at all? Isn't this only a matter of efficiency?}
In fact, we plot the number of extra retransmissions against the loss rate in Figure~\ref{fig:seq-rewrite-rtx-rate}, and observe that the number is extremely small at loss rates even up to 20\%.

Rewriting sequence numbers in this way is useful not only for SFU-based applications like videoconferencing and cloud gaming, but also for applications where an intermediate server is in charge of selectively forwarding packets from a single transport flow to a receiver, based on its capabilities. For example, if the network performance is poor, a middlebox may choose to suppress ad frames in a video stream.
% \sata{
% Sensor networks
% Selective forwarding of ads
% ML transmission of weights
% In general: need to write seq. numbers when there is a clear hierarchy across packet types / rewritign process needs to be transparent to the receiver in order to still enable NACKs/retransmissions}
% \joon{I think we need a diagram to show this. Seems interesting enough, but it is hard to follow by just reading text.}

\subsection{Switch as a Server}
\label{subsec:as-server}

In addition to performing the tasks mentioned above, the \sys{} data plane has its own IP address and MAC addresses (associated with the interfaces it receives and transmits traffic from). It responds to ARP requests and ICMP echo requests and listens on a particular "SFU" port, thus behaving as a server for external hosts.



==> sec/archive/discussion.tex <==
% !TEX root = ../p4-sfu-nsdi24.tex  

\section{Discussion}
\label{sec:discussion}

\noindent
\textbf{Hardware-amenable wire protocols.}~%
The WebRTC framework and its protocols, which most video-conferencing applications follow, are not hardware-friendly. 
This is because the protocol was initially designed as a P2P protocol, where software 
with complex algorithms is designed to run on end-host devices. Furthermore, codec
and protocol designers emphasize efficiency, making every bit count and aiming to minimize the bandwidth usage between participants. This is a noble goal, but makes the protocol inherently challenging to parse and process in hardware (e.g., network devices). In particular, the complex compression algorithm and dynamic variable-length header fields make parsing and processing challenging, even with programmable data planes. 
Following the trend of hardware offloading and co-designing software and hardware, it is worth re-exploring the design and implementation of more hardware-amenable protocols, shifting the balance towards offloading computation and less on bandwidth optimization. In fact, the community has seen ideas in the past, for example using fixed-length header fields in BGP routing~\cite{kiyak:hair}.\\
%
\noindent
\textbf{Encryption and message authentication.}~%
Privacy and security of video-conferencing applications are important, which are upheld by end-to-end encryption and message authentication through symmetric/asymmetric encryption systems and cryptographic hash functions. Yet, running such complex algorithms and functions in a programmable data plane at line rate is non-trivial. Due to this challenge, our working prototype does not perform encryption and message authentication (e.g., attaching re-calculated Message Authentication Code, or MAC to a packet). However, this limitation is not fundamental. There has been notable work in performing encryption/decryption and cryptographic hash functions in programmable data planes~\cite{oliveira2021dh,chen2020implementing,schulz2023cryptographic,scholz2019cryptographic,wang2023raven}, and recent SmartNICs have even more advanced capabilities~\cite{kim2020case,kottur2022implementing,taranov2020srdma}. Furthermore, the switch does not need to process the payload. As a result, an entirely encrypted payload is fine as long as headers are in clear text. Rewriting header fields, as required by our system, however makes computing new MACs necessary. These codes are computed over the relatively short RTP header. Designs such as the one reference above as well as co-located cryptographic processors could take over this tasks if packets need to be changed.\\
%
\noindent
\textbf{SFU cascading.}~%
Selective Forwarding Unit (SFU) cascading is a technique of deploying SFUs in a hierarchical manner to improve the scalability of the infrastructure that supports video-conferencing applications by aggregation of media streams at higher-level SFUs. We argue our system is not an alternative to or a competing solution with SFU cascading. In fact, the approaches are independent and could be combined to improve the scalability further. Our control/data plane split has the potential to simplify deploying many SFU data planes under the management of a single controller. Our current system is already designed in this way and would provide the architectural framework to enable such SFU topologies.\\
%
\noindent
\textbf{SmartNIC as an alternative target.}~%
Given the stronger computational capability and flexibility, including the ability to run more advanced cryptographic functions, SmartNICs are a promising alternative target in place of programmable switches like the Intel Tofino~\cite{intel:tofino}. Of course, port density and data rate are issues for SmartNIC-based solutions as traffic and infrastructure scale up. Regardless of the target, our work presents an excellent division of labor to support large video-conferencing traffic loads, where packet processing-heavy tasks are offloaded to hardware.\\

==> sec/archive/dissecting.tex <==

\section{Dissecting Selective Forwarding Units}
\label{sec:dissect}

Before introducing our system, we present the high-level challenges that SFUs solve, followed by a characterization of the exact packet-level functionality SFUs provide using real-world, passively collected traces of Zoom traffic from our campus network which we analyze using the methods and tools presented in~\cite{michel:passive-measurement-zoom}.
We also use data from the Zoom API provided by our IT department.

\subsection{Selective Forwarding Units (SFUs)}

% \begin{figure}[t]
%     \centering
%     \begin{minipage}[t]{0.49\textwidth}
%         \includegraphics[width=\columnwidth]{fig/call-arch.pdf}
%         \caption{Peer-To-Peer (P2P) vs. Selective Forwarding (SFU). Each Color Represents a Media Stream.}
%         \label{fig:call-arch}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t]{0.49\textwidth}
%         \includegraphics[width=\columnwidth]{fig/sfu-operation.pdf}
%         \caption{Media-Forwarding Operation of an SFU using Scalable Video Coding.}
%         \label{fig:sfu-operation}
%     \end{minipage}
%     \vspace{-0.3cm}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{fig/call-arch.pdf} % for 2-column layout
    % \includegraphics[width=0.45\columnwidth]{fig/call-arch.pdf} % for 1-column layout
    \caption{Video-Conferencing Architectures: Peer-To-Peer (P2P) vs. Selective Forwarding (SFU). Each Color Represents a Participant's Media Stream.}
    \label{fig:call-arch}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\columnwidth]{fig/sfu-operation.pdf} % for 2-column layout
    % \includegraphics[width=0.45\columnwidth]{fig/sfu-operation.pdf} % for 1-column layout
    \caption{Media-Forwarding Operation of an SFU using SVC.}
    \label{fig:sfu-operation}
\end{figure}

Traditionally, Internet telephony and video-conferencing applications have been based on a peer-to-peer (P2P) architecture where each participant sends and receives media streams to and from every other participant~\cite{baset:analysis-of-skype}.
Direct P2P connections between meeting participants result in the lowest latency between two given clients but can be challenging to realize in the presence of firewalls and network address translators (NAT)~\cite{ice-rfc,ford:p2p-across-nat}.
The left side of Figure~\ref{fig:call-arch} depicts the media streams in a three-party P2P meeting.
As each sender sends an individual media stream per other participant, this approach requires substantial uplink bandwidth which is often not available in residential and wireless Internet access settings.
As a result, most VCAs use P2P connections only for some two-party calls (e.g., Zoom) or not at all (e.g., Google Meet)~\cite{nistico:comparative-study-rtc, michel:passive-measurement-zoom, lee:demystifying-vca}.

To avoid the uplink bottleneck problem, selective forwarding units were introduced that forward media streams among clients and are the de-facto standard in video conferencing today.
Similar intermediate servers are used for live-streaming use cases~\cite{whip-whep-live-streaming}.
The topology in terms of media streams of a three-party SFU-based meeting is depicted on the right side of Figure~\ref{fig:call-arch}.
An SFU receives each client's media streams, replicates the streams for each downlink participant and forwards the media accordingly.
In addition to forwarding media, SFUs must adapt media streams for the network conditions, device capabilities, or preferences of individual downstream participants.

While the use of SFUs solves the problem of constrained uplink bandwidth and reduces the required CPU resources at clients, SFUs do not entirely solve the scalability problem in multi-party video conferencing as sometimes suggested~\cite{webrtc-arch-basics-blog}.
It is important to note that the number of streams that are required in an SFU scenario still grows quadratically with the number of participants.
There are $N^2$ media streams for $N$ participants (per media type in use) in an SFU topology which even grows slightly faster compared to the $N(N-1)/2$ streams in a P2P topology.
%(see Figure~\ref{fig:call-arch}).
The key difference is that all these streams are now sent to or received by the SFU, effectively moving the bottleneck from the clients to the SFU.

The second important observation is that the amount of work that an SFU needs to perform is determined by the number of streams and not by the number of participants which therefore leads to a quadratic scaling behavior at the SFU.
This is due to the fact that every incoming stream needs to be replicated for each of the downstream participants and then sent out accordingly (see Figure~\ref{fig:sfu-operation}).
At hundreds of packets (typically between 800 and 1400 Bytes in size for video and around 200 Bytes in size for audio) per second per stream, this requires copying significant amounts of data among socket buffers for receiving packets and before sending them out, resulting in high CPU load and frequent context switching.

\subsection{SFUs as Packet Processors}

Selective forwarding units implement two key functionalities. First, they forward media streams from every participant to every other participant. Second, they reduce the bitrate forwarded to individual participants in response to congestion or device capabilities.
The naive way of implementing an SFU is to leverage a split-proxy design that terminates a WebRTC peer connection, passes the media at the application layer between sockets and repacketizes the signal again.
This would result in different packet sizes, possibly different payload ciphertext if packets are re-encrypted, and also different header fields (e.g., timestamps, sequence numbers, stream identifiers).

Analyzing Zoom packet traces collected on our campus, however, we observed that Zoom's SFUs do not perform any modification of the packets; they do not change header fields, do not translate sequence numbers, nor do they change the packet's encrypted payload in any way.
The same results have been reported in~\cite{michel:passive-measurement-zoom} where this insight is used to infer the number of participants in a given meeting.
Consequently, the forwarding operation of an SFU reduces to replicating a packet $N-1$ times for a meeting with $N$ participants and sending the resulting $N-1$ packets to the respective participants.
Taking this into consideration, the question arises how these SFUs are even able to modify the quality (and consequently the bitrate) of a media stream for a specific downstream participant.
%\joon{Reviewer is left with a question here, but the next paragraph starts to explain something else. Reviewer might feel 'hmm? are you going to answer the question?' Turns out, the next paragraph *is* to answer the question, but that only becomes clear after three more paragraphs. Can we make the intention of the next paragraph clearer?}
% To understand this rate adaptation mechanism from the network perspective, we again collected packet-level traces of Zoom traffic in our campus network which we analyzed 

We now answer this question by analyzing a real-world meeting with 19 participants on our campus interconnected through a Zoom SFU that took place in May 2022.
Figure~\ref{fig:kbits-per-stream} shows an example of a participant's outgoing video stream and the corresponding incoming streams at two other participants.
Time zero denotes the start of the meeting at which the sending participant starts transmitting a low-bitrate video stream which then increases in bitrate at around 20 seconds into the meeting.
Presumably in response to constrained downlink capacity, the SFU then reduces the bitrate forwarded to participant 12 (at around 110s) and the bitrate forwarded to participant 17 (at around 200s), respectively.
%\joon{Are these numbers 12 and 17 important? If not, can we just make them 2,3? Also, the plots have "Receiver" but the text says "Participant." Should be consistent.}

Zoom uses the Real-time Transport Protocol (RTP)~\cite{rtp-rfc} encapsulated in custom, proprietary headers over UDP to transmit media~\cite{michel:passive-measurement-zoom}.
The RTP header carries a sequence number and various extension fields in each packet that is not being changed by Zoom's servers during forwarding.
As a result, we can exactly specify which packets are forwarded to a given participant by the SFU and which are not.
% We further observed that Zoom's RTP packets carry various RTP extension headers.
One header extension field carries a three-byte value that appears to be a bit mask.
The packets in the outgoing media streams typically carry between two and six different values for this field across their packets which we for now denote as the \emph{packet type}.
We observe that the SFU only forwards either all or a strict subset of these packet types to a given participant; sometimes, this subset changes during the meeting.

% \begin{figure}[t]
%     \centering
%     \begin{minipage}[t]{0.45\textwidth}
%         \includegraphics[width=\columnwidth]{fig/kbits-per-stream-1}
%         \caption{Forwarded bytes of a single video stream to two separate participants in a Zoom meeting.}
%         \label{fig:kbits-per-stream}
%     \end{minipage}
%     \hspace{0.5cm}
%     \begin{minipage}[t]{0.45\textwidth}
%         \includegraphics[width=\columnwidth]{fig/kbits-per-layer-1}
%         \caption{Forwarded bytes per scalability layer of a single video stream to a participant in Zoom.}
%         \label{fig:kbits-per-layer}
%     \end{minipage}
%     \vspace{-0.3cm}
% \end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\columnwidth]{fig/kbits-per-stream-1} % for 2-column layout
    % \includegraphics[width=0.6\columnwidth]{fig/kbits-per-stream-1} % for 1-column layout
    \caption{Forwarded bytes of a single video stream to two separate participants in a Zoom meeting.}
    \label{fig:kbits-per-stream}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\columnwidth]{fig/kbits-per-layer-1} % for 2-column layout
    % \includegraphics[width=0.6\columnwidth]{fig/kbits-per-layer-1} % for 1-column layout
    \caption{Forwarded bytes per scalability layer of a single video stream to a single participant in a Zoom meeting.}
    \label{fig:kbits-per-layer}
\end{figure}

Figure~\ref{fig:kbits-per-layer} shows the bit rate of the same media stream as previously shown broken down by packet type.
We can see that the adaptation of the media stream received by participant 17 around second 200 is achieved by changing the set of packet types forwarded to this client.
This is consistent with previous observations that Zoom uses media scalability through Scalable Video Coding (SVC) and Simulcast~\cite{michel:passive-measurement-zoom,how-zoom-works, w3c:webrtc-svc, schwarz:svc-overview} and leverages this field to indicate to the SFU which layer of a scalable stream the respective packet carries.
It is common to encode the type of scalability layer in the RTP header~\cite{schwarz:svc-overview} which is transmitted in clear text; 
similar header extensions exist, for example, for the AV1 codec~\cite{av1, av1-rtp} which we leverage in this work.



The mechanism behind SVC is illustrated in Figure~\ref{fig:sfu-operation}.
Here, the SFU relays a media stream in a four-party meeting where one participant receives a reduced frame-rate stream (15 fps instead of 30 fps) which is achieved by dropping every other frame.
Additionally, media is packetized in such a way that scalability layers do not cross packet boundaries.
The letters A and B here denote the two different scalability layers, a base layer (A) and an enhancement layer (B) which depends on the base layer, as denoted by the black arrows.

We conclude that SFUs can be implemented by replicating packets and sending copies out to all receiving participants.
Furtheremore, if SVC (or the related technology, Simulcast~\cite{lin:gso-simulcast}) is used, adapting a media stream reduces to forwarding a clearly defined and correspondingly labeled subset of packets to a given participant.
%\joon{this part is hard to parse: "..adapting a media stream reduces to forwarding a clearly defined and correspondingly labeled subset of packets to a given participant."}


% \joon{I wonder if we need a *takeaway* paragraph/subsection at the end of Section 2, which will tie well with Section 3. I suppose Section 2 should convince reviewers that "yeah, a data plane might be able to take over many SFU functions here!" But I wonder if some reviewers will miss that because they focused too much on learning about what an SFU is.}

==> sec/archive/eval.tex <==
% !TEX root =  ../p4-sfu-nsdi24.tex

\section{Evaluation}%
\label{sec:eval}



% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\columnwidth]{fig/campus-bw-1.pdf}
%     \caption{Bandwidth Util. of Zoom Calls in Campus Dataset}
%     \label{fig:campus-bw}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\columnwidth]{fig/pct-bw-1.pdf}
%     \caption{Bandwidth Utilization during 2nd week of Feb '23 as Percentage of Device Capacity}
%     \label{fig:pct-bw}
% \end{figure}

In this section, we present the evaluation of \sys{} by first describing the experimental setup (\S\ref{subsec:setup}),
% then demonstrating its core functionality as an SFU (\S\ref{subsec:func-eval}), 
then reporting results on key aspects of the system components (\S\ref{subsec:control-eval}, \S\ref{subsec:data-eval}), and finally analyzing its scalability (\S\ref{subsec:scale-eval}).

\subsection{Experimental Setup}
\label{subsec:setup}

We deploy the data plane of \sys{} on an Intel Tofino hardware switch in our campus testbed with a labeled maximum bandwidth of 3.2 Tbit/s. Our switch agent runs on the CPU of this switch, which is an Intel Pentium CPU equipped with 8 cores and 8 GB memory. The controller is deployed on an Intel Xeon server with 40 CPU cores and 96 GB memory. We use a separate Intel Xeon server with the same configuration to host the meeting participants. Each participant runs in a separate browser tab on this server, and their media streams are uniquely identified by their UDP ports. The Tofino serves both as a switch for forwarding background traffic (including for signaling) between the two servers and also as the SFU for video-conferencing traffic.

% \subsection{SFU Functionality}
% \label{subsec:func-eval}

% \sata{Insert figure of a 4-participant meeting showing data rate in/out and frame rate in/out.}\\
% \sata{If possible, insert figure of a 3-participant meeting with rate adaptation on for one of them.}

\subsection{Control Plane}
\label{subsec:control-eval}



We first analyze the amount of packets and bytes that our controller needs to process compared with the amount of packets that stay entirely in the data plane.
This ratio demonstrates the feasibility of Scallop's control/data-plane split.
The key protocol in video conferencing is the Real-Time Transport Protocol (RTP) which is used to transmit media streams.
RTP uses a fixed-sized base header and a variable number of extension headers to carry additional information about the media stream~\cite{rtp-rfc} which makes it amenable to match-action processing in the data plane.
The RTP header is followed by the actual media payload which is typically encrypted while the header is not.

To get a better understanding of the types of packets and the amount of data that is processed in a typical video-conferencing session, we collected a packet-level trace of three-party meeting using \sys{} where participants send a 720p AV1 video stream using SVC with two temporal layers and an Opus audio stream.
We then analyzed the trace to determine the number of packets and bytes that can be processed in the data plane and the control plane, respectively.
The results of this analysis are summarized in Table~\ref{tab:pkt-types}.

The experiment ran for ten minutes during which we collected a total of 180,718 packets.
We found that 94.5\% of these packets were RTP packets which can be handled in the data plane with the exception of RTP packets containing an extended AV1 dependency descriptor which however only accounted for 5 packets.
RTCP accounted for 5.06\% of all packets and 0.48\% of all bytes.
Our switch agent uses RTCP receiver reports and REMB messages to control the rate-adaptation logic.
These packets accounted for 3.41\% of overall packets.
Finally, STUN packets accounted for 0.38\% of all packets and also need to be processed in software.
In summary, 96.46\% of all packets and 99.65\% of all bytes can be processed in the data plane, making this workload naturally suited for such a control/data-plane split.
Almost more importantly, the remaining packets, with the exception of a few STUN packets at the beginning of each session for connection establishment, are not blocking.

\subsection{Data Plane}
\label{subsec:data-eval}

% \begin{table}[t]
%     \centering
%     \begin{minipage}[b]{0.49\textwidth}
%     \scriptsize
%     \begin{tabular}{p{1.8cm}|p{1.0cm}|p{1.3cm}|p{0.95cm}}
%         \textbf{Resource type} & \textbf{Scaling behavior} & \textbf{under peak campus load (avg.)} & \textbf{under max util. (avg.)} \\
%         % \hline
%         % - Lines of code & Fixed & 2001 & = \\
%         % - Compile time & Fixed & 20.2s & = \\
%         \hline
%         Parsing depth & Fixed & Ing. 27, Eg. 7 & = \\
%         No. of stages & Fixed & Ing. 7, Eg. 5 & = \\
%         PHV containers & Fixed & 17.9\% & = \\
%         Exact xbars & Fixed & 5.66\% & = \\
%         Ternary xbars & Fixed & 2.52\% & = \\
%         Hash bits & Fixed & 4.62\% & = \\
%         Hash dist. units & Fixed & 6.94\% & = \\
%         VLIW instr. & Fixed & 7.29\% & = \\
%         Logical table ID & Fixed & 21.87\% & = \\
%         SRAM & Fixed & 6.77\% & = \\
%         TCAM & Fixed & 1.38\% & = \\
%         \hline
%         \#PRE nodes (opt.) & Linear & 400 & 65,535 \\
%         \#PRE nodes & Quadratic & 800 & 65,535 \\
%         \hline
%         Egress throughput & Quadratic &  1.2 Gb/s & 197 Gb/s \\
%         \hline
%     \end{tabular}
%     \caption{Resource usage of the Tofino data plane.}
%     \label{tab:tofino-usage}
%     \end{minipage}

%     \begin{minipage}[b]{0.49\textwidth}
%     \scriptsize
%     \begin{tabular}{l|rrr|rr} 
%         % \hline
%         \textbf{Type} & \textbf{Packets} & \textbf{Pct.} & \textbf{Per sec.} & \textbf{KBytes} & \textbf{Pct.} \\
%         \hline
%         RTP & 170,870 & 94.5 & 284.30 & 166,762 & 99.47 \\
%          - Audio & 29,746 & 16.46 & 49.49 & 3,826 & 2.28 \\
%          - Video & 141,124 & 78.09 & 234.81 & 162,935 & 97.19 \\
%          \hspace{0.1cm} - AV1 DS* & 5 & $\lll$ & 0.008 & 6 & $\lll$ \\

%         RTCP & 9,153 & 5.06 & 15.22 & 801 & 0.48 \\
%          - SR/SDES & 3,456 & 1.91 & 5.75 & 304 & 0.18 \\
%          - RR* & 240 & 0.39 & 0.13 & 15 & 0.01 \\
%          - RR/REMB* & 5,457 & 3.02 & 9.07 & 482 & 0.29 \\
        
%          STUN*& 695 & 0.38 & 1.15 & 89 & 0.05 \\
%         \hline
%         \textbf{Ctrl. Plane} & 6397 & \textbf{3.54} & 10.64 & 593 & \textbf{0.35} \\
%         \textbf{Data Plane} & 174,326 & \textbf{96.46} & 290.06 & 167,066 & \textbf{99.65} \\
%         \hline
%         Total & 180,718 & 100 & 300.69 & 167,653 & 100 \\
%     \end{tabular}
%     % \vspace{0.1cm}
%     \caption{Packets per participant sent to SFU (10 min.)}
%     \label{tab:pkt-types}
%     \end{minipage}
%     \vspace{-0.3cm}
% \end{table}


\begin{table}[t]
    \centering
    \scriptsize
    \begin{tabular}{p{1.8cm}|p{1.0cm}|p{1.7cm}|p{0.95cm}}
        \textbf{Resource type} & \textbf{Scaling behavior} & \textbf{Usage under peak campus load (avg.)} & \textbf{under max util. (avg.)} \\
        % \hline
        % - Lines of code & Fixed & 2001 & = \\
        % - Compile time & Fixed & 20.2s & = \\
        \hline
        Parsing depth & Fixed & Ing. 27, Eg. 7 & = \\
        No. of stages & Fixed & Ing. 7, Eg. 5 & = \\
        PHV containers & Fixed & 17.9\% & = \\
        Exact xbars & Fixed & 5.66\% & = \\
        Ternary xbars & Fixed & 2.52\% & = \\
        Hash bits & Fixed & 4.62\% & = \\
        Hash dist. units & Fixed & 6.94\% & = \\
        VLIW instr. & Fixed & 7.29\% & = \\
        Logical table ID & Fixed & 21.87\% & = \\
        SRAM & Fixed & 6.77\% & = \\
        TCAM & Fixed & 1.38\% & = \\
        \hline
        \#PRE nodes (opt.) & Linear & 400 & 65,535 \\
        \#PRE nodes & Quadratic & 800 & 65,535 \\
        \hline
        Egress throughput & Quadratic &  1.2 Gb/s & 197 Gb/s \\
        \hline
    \end{tabular}
    \caption{Resource usage of the Tofino data plane.}
    \label{tab:tofino-usage}
        \vspace{-0.3cm}
\end{table}

\begin{table}[t]
    % data and analysis in: /Users/olli/src/research/webrtc-analysis/data/pkt_types
    \centering
    \scriptsize
    \begin{tabular}{l|rrr|rr} 
        % \hline
        \textbf{Proto./Type} & \textbf{Packets} & \textbf{Pct.} & \textbf{Per sec.} & \textbf{KBytes} & \textbf{Pct.} \\
        \hline
        RTP & 170,870 & 94.5 & 284.30 & 166,762 & 99.47 \\
         - Audio & 29,746 & 16.46 & 49.49 & 3,826 & 2.28 \\
         - Video & 141,124 & 78.09 & 234.81 & 162,935 & 97.19 \\
         \hspace{0.1cm} - AV1 DS* & 5 & $\lll$ & 0.008 & 6 & $\lll$ \\

        RTCP & 9,153 & 5.06 & 15.22 & 801 & 0.48 \\
         - SR/SDES & 3,456 & 1.91 & 5.75 & 304 & 0.18 \\
         - RR* & 240 & 0.39 & 0.13 & 15 & 0.01 \\
         - RR/REMB* & 5,457 & 3.02 & 9.07 & 482 & 0.29 \\
        
         STUN*& 695 & 0.38 & 1.15 & 89 & 0.05 \\
        \hline
        \textbf{Ctrl. Plane} & 6397 & \textbf{3.54} & 10.64 & 593 & \textbf{0.35} \\
        \textbf{Data Plane} & 174,326 & \textbf{96.46} & 290.06 & 167,066 & \textbf{99.65} \\
        \hline
        Total & 180,718 & 100 & 300.69 & 167,653 & 100 \\
    \end{tabular}
    % \vspace{0.1cm}
    \caption{Packets per participant sent to SFU (10 min.)}
    \label{tab:pkt-types}
        \vspace{-0.3cm}
\end{table}

\noindent
\textbf{Tofino resource utilization.}
We implement \sys's data plane using $\sim$2000 lines of P4$_{16}$ code. We report the performance of our prototype in Table~\ref{tab:tofino-usage} (the = symbol in the last column implies that the resource usage is same under any setting). We categorize the resource types available on the Tofino by how they scale with the number of participants---they either remain fixed, scale linearly, or quadratically. The high ingress parsing depth is evidence of the flexible, recursive parsing we describe earlier in Section~\ref{sec:data}. The number of stages consumed by our program falls squarely within the bounds of the maximum available on the Tofino, leaving ample opportunity for a network developer to deploy additional applications on it. For the rest of the components with fixed scaling behavior, we report the average utilization across all stages. Again, we observe that the resource usage is low enough such that other network applications can be comfortably deployed in conjunction with \sys.

For the components with variable resource utilization, we report their usage under two conditions. First, we report the usage under the peak load observed in our campus network during a month, which was $\sim$400 concurrent active participants. Second, we report the usage under the maximum number of participants supported by our Tofino implementation when the PRE resources are exhausted (more analysis in \S\ref{subsec:scale-eval}), which is $2^{16}$. The numbers are based on the assumption of three participants per meeting---which is the median we observed in our campus trace---all sending media concurrently. As explained in Section~\ref{sec:data}, our PRE resources scale linearly with the number of participants when the optimized strategy is used, and is equal to the number of concurrently active participants. When the optimization is not used, the scaling is quadratic (and results in double the utilization). The required egress bandwidth always scales quadratically, since all the replicated packets need to be processed by the egress pipeline.
%
\noindent
\textbf{Overhead due to sequence number rewriting.}
In Figure~\ref{fig:seq-rewrite-rtx-rate}, we report the overhead of our sequence number rewriting heuristic described in Section~\ref{sec:data}. This overhead is in terms of the fraction of extra retransmissions triggered by the receiver due to a mismatch between the rewritten sequence number and the ideal rewritten sequence number an oracle may have generated. We observe that the overhead is below 5\% for up to 10\% loss rate, and around 7.5\% for a 20\% loss rate. Even under really high loss rates (where the meeting itself would start to become unusable), the overhead does not exceed 20\%.

% \begin{figure}[t]
%     \centering
%     \begin{minipage}[t]{0.45\textwidth}
%         \includegraphics[width=\columnwidth]{fig/seq-rewrite-rtx-rate-1.pdf}
%         \caption{Erroneous Retransmissions when Rewriting Sequence Numbers in Data Plane.}
%         \label{fig:seq-rewrite-rtx-rate}
%     \end{minipage}
%     \hspace{0.5cm}
%     \begin{minipage}[t]{0.45\textwidth}
%         \includegraphics[width=\columnwidth]{fig/switch-agent-bw-1.pdf}
%         \caption{Bytes processed during 2nd week of Feb '23}
%         \label{fig:switch-agent-bw}
%     \end{minipage}
%     \vspace{-0.3cm}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{fig/seq-rewrite-rtx-rate-1.pdf} % for 2-column layout
    % \includegraphics[width=0.45\columnwidth]{fig/seq-rewrite-rtx-rate-1.pdf}
    \caption{Erroneous Retransmissions when Rewriting Sequence Numbers in Data Plane.}
    \label{fig:seq-rewrite-rtx-rate}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{fig/switch-agent-bw-1.pdf} % for 2-column layout
    % \includegraphics[width=0.45\columnwidth]{fig/switch-agent-bw-1.pdf}
    \caption{Bytes processed during 2nd week of Feb '23}
    \label{fig:switch-agent-bw}
\end{figure}


\subsection{Scalability}
\label{subsec:scale-eval}



\noindent
\textbf{Bytes processed by the switch agent.}
As we explained in Section~\ref{subsec:control-eval}, only a tiny fraction of packets and bytes are processed in software when \sys{} is used, as opposed to a software-based SFU. Figure~\ref{fig:switch-agent-bw} makes this point visually, where the blue curve shows the byte rate a software-based SFU would have to process if it were to handle all of our campus traffic during a week (peaks around 1250 Mbit/s), and the red curve shows the byte rate that the Scallop switch agent would have to process in comparison (peaks around only 4.4 Mbit/s). Even for a powerful 40 Gbit/s server, the peak byte rate from our campus already consumes 3.1\% of its total capacity if a software-based SFU is used. For large providers like Zoom, many such servers would, therefore, be required to serve the thousands of campuses and enterprises that use their services. In contrast, with Scallop, only 0.01\% of the server's capacity would be used.\\
%
\noindent
\textbf{Maximum PRE utilization.}
In Figure~\ref{fig:pre-lim}, we show the maximum number of meetings that can be supported by the Tofino's PRE as the meeting size (i.e., the number of participants per meeting) increases. The dotted lines correspond to a non-optimized version of our PRE usage where the resource utilization scales quadratically with the number of active participants. In contrast, the solid green line shows this variation when the optimized version is used. The purple curve corresponds to the scenario where only 1 participant sends media in a meeting, however large the meeting size; it forms the upper bound of the number of meetings supported by our non-optimized PRE. The blue curve corresponds to the lower bound instead, where all the participants are always sending media. The red curve shows a scenario where 5 participants send media, which is perhaps more representative of a meeting in the wild (rather than, for example, all 100 people sending media in a meeting with 100 participants).

We observe that when meeting sizes are larger than $\sim$80 and all participants send, the non-optimized PRE can only handle 10 meetings or less. In contrast, the optimized version scales linearly with the total number of participants, irrespective of the meeting composition, and performs almost as well as the lower bound case with the non-optimized PRE. Even for meetings with 100 participants, the optimized PRE can handle close to 1000 such meetings.\\
%
\noindent
\textbf{Tradeoff between PRE resources and egress bandwidth.}
Figure~\ref{fig:perf-env} shows the "performance envelope" of the Tofino, where we analyze the tradeoff between the PRE resources (which is also equal to the total number of concurrent participants served by \sys{} when the optimized version is used) and the bandwidth of the Tofino. The dotted square represents the range of possible tradeoff points between these resources. Since bandwidth scales quadratically with meeting size, we observe that as the meeting sizes go higher, the bandwidth rises more sharply, until for meetings larger than around 30 participants (all sending simultaneously), the labeled bandwidth of the Tofino gets exhausted first, before the resource limit on the PRE (i.e., $2^{16}$) is reached.

\begin{figure}[t]
    \centering
    \begin{minipage}[t]{0.45\textwidth}
        \includegraphics[width=\columnwidth]{fig/pre-lim-1.pdf}
        \caption{Max. Meetings supported by Tofino at max. PRE Utilization}
        \label{fig:pre-lim}
    \end{minipage}
    \hspace{0.5cm}
    \begin{minipage}[t]{0.45\textwidth}
        \includegraphics[width=\columnwidth]{fig/perf-env-1.pdf}
        \caption{Tradeoff between Tofino PRE Resources and Throughput}
        \label{fig:perf-env}
    \end{minipage}
        \vspace{-0.3cm}
\end{figure}


% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=0.9\columnwidth]{fig/pre-lim-1.pdf} % for 2-column layout
%     \includegraphics[width=0.45\columnwidth]{fig/pre-lim-1.pdf}
%     \caption{Max. Meetings supported by Tofino at max. PRE Utilization}
%     \label{fig:pre-lim}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=0.9\columnwidth]{fig/perf-env-1.pdf} % for 2-column layout
%     \includegraphics[width=0.45\columnwidth]{fig/perf-env-1.pdf}
%     \caption{Tradeoff between Tofino PRE Resources and Throughput}
%     \label{fig:perf-env}
% \end{figure}
%




\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/outgoing-fps-1}
        \caption{Send Frame Rate}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/incoming-fps-1}
        \caption{Receive Frame Rate}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/incoming-bitrate-stack-1}
        \caption{Receive Bit Rate at Part. 3}
    \end{subfigure}
    \caption{Example of \sys-Based Rate Adaptation: Participant 3's Receive Bitrate is Reduced Twice.}
    % \vspace{-0.4cm}
\end{figure*}



==> sec/archive/intro1.tex <==
% !TEX root =  ../p4-sfu-nsdi24.tex

\section{Introduction}%
\label{sec:intro}

% sheer volume of VCA traffic up and also more heterogenous devices and network characteristics

Over the past years, video-conferencing applications (VCA) have become \textcolor{blue}{essential for a wide range of organizations}, including business enterprises, healthcare facilities, and educational institutions.
The current and expected growth of these applications~\cite{feldmann:lockdown-effect, video-conf-market} require an unprecedented scale of their complex underlying infrastructure.
This particularly concerns the infrastructure and servers that applications like Google Meet~\cite{google-meet}, Microsoft Teams~\cite{ms-teams}, and Zoom~\cite{zoom} require to relay real-time audio or video traffic among meeting participants.
These servers are called selective forwarding units (SFUs) and are the backbone of modern video-conferencing applications~\cite{gouaillard:webrtc-sfu-load-test,jitsi-videobridge,mediasoup,lopez:kurento}.
Despite the importance of this core infrastructure, the majority of research in this area has focused on the other stakeholders in the video-conferencing ecosystem with work on the end-user side in the form of novel video codecs~\cite{zhang:loki, fouladi:salsify, schwarz:svc-overview}, rate-adaptation algorithms~\cite{carlucci:google-cc, decicco:cc-for-webrtc, engelbart:cc-for-real-time-over-quic, rfc8698}, measurement studies focusing on meeting quality~\cite{bronzino:inferring-video-quality,michel:passive-measurement-zoom, chang:can-you-see-me, macmillan:perf-video-conferencing}, as well as work on the role of network operators~\cite{janczukowicz:specialized-net-servies-webrtc, elmokashfi:geography-matters}.
This leaves the VCA operator's side, issues in the underlying infrastructure, and the pivotal role of selective forwarding units less explored.
% At the same time, these systems must also increasingly support a wide range of client devices (e.g., mobile phone vs. desktop) and network types and conditions (e.g., cellular vs. wired broadband) as well as rapidly changing network conditions within a single meeting.

% introduce SFUs, provide short background, and summarize challenges

% Today, selective forwarding units (SFU) implemented in software on general-purpose servers perform the task of relaying media streams among participants and adjusting them for the individual participants and network conditions, constituting the backbone of modern video-conferencing and live-streaming systems~\cite{gouaillard:webrtc-sfu-load-test,jitsi-videobridge,mediasoup,lopez:kurento}.


These servers must be able to sustain increasingly high data rates due to growing adoption and quality expectations and dynamically scale up and down to accommodate the varying number of meetings, participants, and dynamics within a meeting (i.e., when participants start or stop sharing audio or video).
Furthermore, SFUs must support logic to monitor video and audio quality to enable rapid and fine-grained adaptation of media signals to match sender's and receiver's capabilities and quickly react to changing network conditions.
Achieving high performance given the need for such granular control is hard, putting these two properties traditionally at odds~\cite{michel:prog-data-plane,yu:mantis,bosshart:p4} and posing a significant challenge for VCA operators.
Today, in order to provide this level of control, SFUs are implemented in user-space software, forwarding thousands of (often small) UDP packets which is a well-known performance corner case within Linux~\cite{cai:understanding-lxovhs}.

In summary, video-conferencing applications heavily rely on general-purpose compute resources inside data centers for a workload that is predominantly defined by packet forwarding and also exhibits a quadratic scaling behavior (cf. Section~\ref{}).
Instead of further improving the performance of video-conferencing infrastructure through client-based solutions or improvements in software packet processing or better provisioning, in this paper, we propose to fundamentally rethink the design of the core component of video-conferencing systems, the SFU.
Specifically, we show that \emph{rearchitecting} and \emph{decoupling} video-conferencing systems into an efficient and fast data plane in hardware that relays media and a control plane in software that handles remaining, infrequent tasks is feasible and vastly improves performance and scalability.

Our key insight supporting this redesign is that forwarding and adapting media signals in video-conferencing systems is strikingly similar to traditional packet-processing tasks.
By characterizing the operation of Zoom's~\cite{zoom} SFUs (see Section~\ref{sec:scale}), we demonstrate this similarity on one of the largest commercial video-conferencing systems.
For example, relaying a media stream to multiple participants is achieved by replicating packets and sending the replicas out to different destinations while recent advances in multimedia allow adjusting the bitrate of a media stream by dropping a specific subset of its packets.

Redesigning video-conferencing systems in this way while maintaining compatibility with existing standards (in our case WebRTC) and making implementation and deployment on and offload to today's line-rate network devices feasible is far from trivial and resulted in several challenges.
In this paper, we describe how to overcome these challenges and present Scallop, a predominantly hardware-based selective forwarding unit that vastly increases the performance of video-conferencing infrastructure.
\sys is implemented on a 3.2 Tbit/s Intel Tofino ASIC and uses a lightweight control plane that handles infrequent tasks and resides on the switch CPU.
With this split, we can handle around 96\% of video-conferencing packets (99\% of Bytes) entirely in hardware, increasing scale and reducing artifacts of software processing, such as jitter, a key performance problem in real-time applications.

To implement \sysnospace, we rearchitected one of the most-widely used video-conferencing platforms (WebRTC) to be split into a control and data plane.
Specifically, we propose strategies to use WebRTC peer connections that allow for an intermediate processor (here SFU) while keeping all media signals valid and feedback signals consistent despite the fact that WebRTC is inherently designed as a peer-to-peer application.
Within the data plane, we propose a set of primitives that taken together implement the core functionality of an SFU but are also applicable in other application-centric networking tasks.

For example, we realize selective application-layer multicast using the Tofino's packet-replication engine (PRE) that adjusts the quality of  media signals on a per-participant basis.
This is realized through dissecting the topology of video conferences into sets of multicast trees and applying selective tree pruning in order to forward a specific frame rate or resolution.
\sys also rewrites sequence numbers in the presence of both intentionally discarded packets and network loss without using a buffer or knowledge about previous or later packet types and instead uses contextual application-layer information to compute the next sequence number.
Finally, we parse deep into the application layer of packets and discuss how parsers can be designed to accommodate for dynamic packet headers.
These capabilities traditionally require software processing driving up per-packet cost and impacting end-to-end performance.


We implemented \sys{} using P4 on a 3.2 Tbit/s Intel Tofino ASIC. Crucially, when replaying campus-scale Zoom traces, we observe that \sys{}'s data and control split results in 96\% of video conferencing packets (and 99\% of overall bytes) being processing \emph{entirely} in hardware. Importantly, synchronous processing of media packets is exclusively handled in the data plane. Consequently, \sys can support up to 65,536 concurrent meeting participants on a single switch, an improvement of 20-40$\times$ over a 32-core commodity server, while avoiding software processing artifacts on key performance metrics such as jitter. We will release \sys{} post publication.



% The majority of work that a SFU performs are therefore functions that network devices are primarily designed for and already efficiently implement.
% We furthermore observed that the workload of an SFU consists of frequent simple operations (i.e., relaying and selectively dropping packets) and infrequent more complex ones (i.e., handling signaling and running rate-adaptation logic).
% Many packet-processing tasks exhibit this property which has been harnessed for years in router design and software-defined networking (SDN)~\cite{feamster:road-to-sdn}.



% VCA infrastructure relatively unexplored

% Despite the importance of these infrastructure components that VCA providers operate, the majority of research in this area has focused on the other stakeholders in the video-conferencing ecosystem.
% Specifically, there has been work on the end-user side in the form of novel video codecs~\cite{zhang:loki, fouladi:salsify, schwarz:svc-overview}, rate-adaptation algorithms~\cite{carlucci:google-cc, decicco:cc-for-webrtc, engelbart:cc-for-real-time-over-quic, rfc8698}, measurement studies focusing on meeting quality~\cite{bronzino:inferring-video-quality,michel:passive-measurement-zoom, chang:can-you-see-me, macmillan:perf-video-conferencing}, as well as work on the role of network operators~\cite{janczukowicz:specialized-net-servies-webrtc, elmokashfi:geography-matters}.
% \textcolor{blue}{This leaves the VCA operator's side, issues in the underlying infrastructure, and the pivotal role of selective forwarding units less explored.}
%\sata{Wonder if this claim sounds too strong, given there are some papers from the VCA operator's perspective (e.g., the GSO Simulcast paper from Alibaba in SIGCOMM'22).} \oliver{I think that ``less explored'' is fair to say but let's see if we can find better wording.}

% While software provides virtually unlimited programmability, it is notoriously challenging and expensive to scale software to such bandwidth-heavy applications~\cite{cai:understanding-lxovhs, hoiland-jorgensen:xdp, jeong:mtcp, abranches:getting-back}.
% Provisioning and scaling these servers is particularly challenging and costly for three reasons.
% First, the amount of work a SFU has to perform is determined by the number of media streams it needs to handle which grows quadratically with the number of participants in a meeting, leading to inherently poor scalability.
% Second, meetings are highly dynamic in nature; participants can join and leave a meeting and decide to share a media signal (e.g., turn on their webcam) at any time. 
% Third, the quadratic scaling behavior together with hard-to-predict meeting dynamics can easily lead to situations where the addition of even a single participant immediately exceeds the server's resources, causing high jitter and packet loss, directly compromising Quality of Experience (QoE)~\cite{bronzino:inferring-video-quality}.
% Since migrating meetings in real time is difficult, the consequence of these issues is that operators need to leave sufficient slack capacity which incurs high operational cost. \sata{I like this paragraph a lot! Wonder if we should forward reference the motivation section here.}
% % Migrating meetings in real time is difficult and, as a result, leaving sufficient slack capacity becomes necessary, incurring high operational cost.

% scalability challenges

% \textcolor{blue}{In particular, provisioning and scaling SFUs is challenging for VCA operators.}
% We observe that the amount of work a SFU has to perform is not linear in the number of participants but is rather determined by the number of media streams it receives and transmits which grows quadratically with the number of participants in a meeting, leading to inherently poor scalability.
% In addition to sharing similar workload dynamics with other user-facing services (e.g., diurnal access patterns), the individual video-conferencing sessions are highly dynamic in nature such that the number of streams is hard to predict and can change rapidly as participants can join and leave a meeting and decide to share a media signal (e.g., turn on their webcam) at any time.
% As a result, the quadratic scaling behavior, hard-to-predict meeting dynamics, and the varying demand in terms of overall meetings can easily lead to situations where the addition of even a single participant immediately exceeds the server's resources, causing high jitter and packet loss, directly compromising Quality of Experience (QoE)~\cite{bronzino:inferring-video-quality}.
% \textcolor{blue}{Through a measurement study using an open-source SFU (Mediasoup), we demonstrate the detrimental effect to QoE when these systems are underprovisioned (see Section~\ref{sec:scale}).}


% Moreover, provisioning and scaling SFUs is particularly challenging for two reasons.
% First, the amount of work a SFU has to perform is not linear in the number of participants but is rather determined by the number of media streams it receives and transmits which grows quadratically with the number of participants in a meeting, leading to inherently poor scalability.
% Video-conferencing sessions are highly dynamic in nature such that the number of streams is hard to predict and can change rapidly as participants can join and leave a meeting and decide to share a media signal (e.g., turn on their webcam) at any time.
% Second, the quadratic scaling behavior together with hard-to-predict meeting dynamics can easily lead to situations where the addition of even a single participant immediately exceeds the server's resources, causing high jitter and packet loss, directly compromising Quality of Experience (QoE)~\cite{bronzino:inferring-video-quality}.


% which incurs high operational cost or under-provision which directly affects meeting quality (more in Section~\ref{sec:scale}).

% problem summary: need high throughput and fine-grained adaptation, today in software, trade off
% Taken together, video-conferencing infrastructure must be able to sustain increasingly high data rates and dynamically scale up and down while also supporting logic that enables rapid and fine-grained adaptation of media streams.
% % to changes in network conditions as well as user behavior.
% Achieving high performance given the need for programmability and granular control is hard, putting these two properties traditionally at odds~\cite{michel:prog-data-plane,yu:mantis,bosshart:p4}.
% To overcome this problem and to support the continuing growth of real-time communication services, in this paper, we advocate to rethink and redesign video-conferencing infrastructure with performance and scalability in mind.

% Consequently, since it is virtually impossible to perfectly provision this infrastructure due to the dynamic character of the workload and the difficulty of migrating interactive meetings in real time, VCA operators are left with two options: 
% they either need to follow a proactive approach by vastly over-provisioning their infrastructure in order to compensate for the various hard-to-predict dynamics of this workload which incurs high operational cost or they end up jeopardizing meeting performance and QoE when trying to reactively scale in response to demand.

% \textcolor{blue}{
% In this paper, instead of incrementally resolving this conundrum through client-based solutions or better provisioning schemes, we propose to fundamentally rethink the design of the underlying infrastructure of video-conferencing systems.
% Specifically, we show that \emph{rearchitecting} and \emph{decoupling} video-conferencing systems into an efficient and fast data plane in hardware that relays media and a control plane in software that handles remaining, infrequent tasks is feasible and vastly improves performance and scalability.}
% % For this, we leverage principles from a long line of work on software-defined networking (SDN) and programmable data planes~\cite{feamster:road-to-sdn}.}

% % the consequence of these issues is that operators either need to over-provision, incurring high cost, or jeopardize QoE (see Section~\ref{sec:scale}).

% % insight: SFU task similar to what net. devices anyways do + workload can be partitioned

% Our key insight supporting this redesign is that forwarding and adapting media signals in video-conferencing systems is strikingly similar to traditional packet-processing tasks.
% \textcolor{blue}{By characterizing the operation of Zoom's~\cite{zoom} SFUs (see Section~\ref{sec:scale}), we demonstrate this similarity on one of the largest commercial video-conferencing systems.}
% For example, relaying a media stream to multiple participants is achieved by replicating packets and sending the replicas out to different destinations while recent advances in multimedia allow adjusting the bitrate of a media stream by dropping a specific subset of its packets.
% ; both packet replication and dropping are key functionalities of networking equipment.
% Moreover, the operation of SFUs can be partitioned into a simple media-forwarding plane that relays and selectively drops media packets based on rules and a control plane that analyzes feedback messages, makes rate-adaptation decisions, and implements connection signaling and establishment.
% The majority of work that a SFU performs are therefore functions that network devices are primarily designed for and already efficiently implement.
% We furthermore observed that the workload of an SFU consists of frequent simple operations (i.e., relaying and selectively dropping packets) and infrequent more complex ones (i.e., handling signaling and running rate-adaptation logic).
% Many packet-processing tasks exhibit this property which has been harnessed for years in router design and software-defined networking (SDN)~\cite{feamster:road-to-sdn}.
% Accordingly, our design also leverages this property to split the workload between software and hardware components.

% Furthermore, the overall workload can be partitioned into frequent simple operations and infrequent complex ones, an insight that applies to many packet-processing tasks and has been harnessed for years in router design and software-defined networking (SDN)~\cite{feamster:road-to-sdn}. 
%\sata{I feel like the "In summary ..." sentence already captures the entire essence of this paragraph pretty neatly, and we may want to trim down the first part of the paragraph.}

% proposal + advantages

% Despite the similarity between the tasks that a SFU and a network switch perform, it is almost surprising that today SFUs are exclusively implemented as monoliths in general-purpose servers, incurring high per-packet cost.

% Based on these insights and following a long line of work on SDN, we argue that video-conferencing systems should be \emph{rearchitected} and \emph{decoupled} into a simple and fast data plane that relays media traffic and a control plane that handles all remaining, infrequent tasks.
% This approach has several advantages.
% Our proposal, following a long line of work on programmable data planes and SDN, has several advantages.
% % Decoupling real-time communication control and data planes has three main advantages.
% First, the data plane can run on special-purpose hardware, such as programmable ASICs or FPGAs, greatly improving performance and reducing cost.
% % Unlike legacy network equipment, these next-generation devices can implement more complex logic and also operate on application-layer protocols, such as RTP and RTCP for real-time multimedia.
% Second, a control plane that interacts with the data plane through a simple API can be used to implement custom control logic, rate-adaptation algorithms, and ultimately enables innovation in the core infrastructure of VCAs.
% Third, a disaggregated architecture also simplifies deploying hierarchies of SFUs where individual units can be placed closer to clients (e.g., at a campus edge or as part of a 5G RAN), shortening the feedback loop and allowing for rapid adaptation.
% Such hierarchical SFUs also reduce the amount of replicated traffic often sent over long distances when multiple participants are geographically co-located but distant from the SFU's location by enabling more efficient multicast topologies.

% challenges

% Redesigning video-conferencing systems in this way while maintaining compatibility with existing standards (in our case WebRTC) and making implementation and deployment on today's network devices feasible is far from trivial and resulted in three specific challenges that we overcome in this paper.

% First, starting from a split between data and control planes of a SFU implementation, it is not obvious how to translate the rich semantics of a video-conferencing session (e.g., participants joining, sharing specific media types, or receiving a specific quality setting of a stream) to data-plane rules that can be implemented in match-action tables in the forwarding pipeline or policies within the queuing engine of a line-rate switch.
% For this, we introduce a translation layer that bridges the semantic gap between the signaling protocol and user behavior and the forwarding rules in the data plane.
% This component which resides on the switch CPU allows implementing SFUs in a disaggregated fashion.

% Second, even with forwarding and replication implemented in the data plane, the packet format and packet semantics used in video conferencing are complex and not designed with hardware processing in mind.
% RTP and RTCP can have complex variable-length header formats to, for example, encode dependencies between frames that are specific to the respective video codec.
% Processing such information within the rigidity of line-rate devices requires clever ways of parsing headers, keeping state, and leveraging the limited programming model.
% For example, our hardware implementation rewrites sequence numbers and keeps track of quality layers and their dependencies in the scalable video stream and uses these data for forwarding decisions at line rate.

% Third, our system heavily uses the queuing and replication engine of the switch in a novel way to selectively forward instead of replicating and then selectively dropping packets.
% % Naively using the replication engine would quickly exhaust the available resources and limit the total number of calls that can be supported.
% This requires synthesizing many different multicast trees per meeting which if done naively would also quickly exhaust the available resources and limit the total number of calls that can be supported.
% The queuing and replication engine is also heavily constrained, but in different ways than other (memory) resources on the device.
% We present a space-optimization strategy that saves resources within the queuing engine of a commercial line-rate switch (i.e., the Intel Tofino), a component that is not commonly highlighted and optimized in the literature.
% Our approach is not specific to an SFU use case but can be applied to other applications that require efficient replication and queueing of packets, such as generic multicast engines.

% C1:
% - starting from split, not clear how to split workload that is traditionally monolithic
% - rich semantics of video conferencing, unlike in other SDN settings with clearer abstraction of communication flows and rules even in application layer (think firewall)
% - required deep analysis of different components, their interactions, messages interchanged, protocols and packet formats used
% - need to translate rich meeting semantics into match-action rules and configurations for the packet processing pipeline and queuing engine, exact split not obvious required deep
% - introduce translation layer between the two significantly different domains

% C2:
% - data plane now needs to operate on protocols that are higher up in stack and semantically richer than typical wire protocols packet processing is done on (e.g., IP or even TCP)
% - here complex extensions that are typically handled in software (e.g., analyzing dependencies between frames based with rich semantics of video codecs)
% - need to fit into programming model of line rate devices

% C3:
% - component that this design is particularly dependent on is the queuing and replication engine
% - something not commonly leveraged, discussed, and optimized in literature
% - however, similar to other resources also heavily constrained, limiting the total number of calls etc. that can be supported
% - so, present strategies to optimize resource usage within PRE of a commercial switch by reusing multicast trees etc.
% - works for other applications that require efficient replication and queueing of packets, such as generic multicast implementations (load balancers, what else?)



% Redesigning video-conferencing systems in this way while maintaining compatibility with existing standards (in our case WebRTC) and making implementation and deployment on today's network devices feasible is far from trivial and resulted in three specific challenges that we overcome in this paper.
% First, finding the most practical split and the interfaces between data- and control-plane components is challenging given the strictly monolithic design of today's systems and frameworks.
% \textcolor{blue}{
% In our design, we use a controller in software that implements the rate-adaptation algorithm and the signaling logic that is required to establish and maintain connections.
% Media streams itself which constitute for the vast majority of packets never traverse the controller and are instead forwarded directly by the data plane.
% }
% Second, unlike in most SDN-controller implementations where there is a clear mapping between control-plane commands and data-plane rules, the rich semantics of video-conferencing sessions with different media types, rate-adaptation mechanisms, and heavy use of (selective) packet replication that need to be represented in the data plane make this mapping less obvious.
% For this, we introduce a custom translation layer that maps video-conferencing semantics (e.g., joining a meeting or muting the microphone) to data-plane rules.
% \textcolor{blue}{
% This component resides directly on the switch CPU and further splits up the controller logic into a centralized, potentially remote, component that manages participants and signaling and a switch-local agent that runs rate-adaptation logic and bridges the semantic gap between the control and data plane.
% }
% Third, processing high-volume media streams and operating on the existing rich protocols and standards used in VCAs inside efficient but resource-constrained programmable hardware is challenging and requires clever ways of leveraging the limited memory and programming model.
% \textcolor{blue}{
% On top of this, our system heavily relies on the switch replication and queueing engine which is also constrained in various ways.
% We present strategies of saving resources within the queuing engine of a commercial line-rate switch (i.e., the Intel Tofino), a component that is not commonly highlighted and optimized in the literature.
% Our approach is not specific to an SFU use case but can be applied to other applications that require efficient replication and queueing of packets, such as generic multicast engines.
% }

% \oliver{Next paragraph is vague: exact challenges TBD.} Redesigning video-conferencing systems in this way is far from trivial.
% First, finding the most practical split and the interfaces between data- and control-plane components is challenging given the strictly monolithic design of today's systems and frameworks.
% Second, processing high-volume media streams and operating on the existing protocols and standards used in VCAs inside efficient programmable hardware is challenging and requires clever ways of leveraging the limited memory and programming model.
% Third, current frameworks and standards like WebRTC, including their requirements and protocols, were originally not designed for large-scale conferencing and follow strict rules (e.g., for key management and connection establishment) that make them difficult to implement in large, cloud-based deployments.
% We believe that many of the design choices and constraints within WebRTC are not necessarily fundamental to its operation or security and argue that some specifications could be relaxed and reframed while ensuring the same functionality, security, and privacy properties in oder to make WebRTC implementations more scalable. \sata{I think this is too defensive and we need not address key sharing in the intro at all, and perhaps delay it until section 2.} \oliver{Agreed, let's postpone writing this paragraph until we are further along in the project.}
% We make recommendations for such changes and also, anecdotally, elaborate on design decisions Zoom has made that depart from WebRTC standards, presumably to improve scalability of their system.

% % contributions

% To summarize, our paper makes two key contributions.
% First, through a measurement study and analysis of Zoom's SFUs, we shed light on the scaling properties of SFUs and the way they are used in a large real-world video-conferencing system.
% We then show how under-provisioned SFUs have a direct impact on video-conferencing QoE and argue that the current monolithic design of these systems is inefficient and inherently hard to scale (Section~\ref{sec:scale}).
% Second, we demonstrate that rearchitecting the core infrastructure for real-time communication systems using SDN principles is feasible, enables more efficient implementations, and results in vastly improved performance and scalability as well as more efficient forwarding topologies, overall lowering operational cost while improving quality (Sections~\ref{sec:arch}, \ref{sec:data}, \ref{sec:control}, and~\ref{sec:eval}).


==> sec/archive/intro2.tex <==
\section{Introduction}%
\label{sec:intro}

Video-conferencing applications (VCAs) such as Google Meet~\cite{google-meet}, Zoom~\cite{zoom}, and Microsoft Teams~\cite{ms-teams} have become essential to individuals and organizations across societal sectors, e.g., business enterprises, healthcare, education, and more. As their popularity surges, so too have their performance requirements, with users mandating high bitrates (video quality), low latency (sub-100ms), and minimal stalls in playback. Unsurprisingly, substantial work has been devoted to improving the performance of VCAs, for example through novel codecs~\cite{zhang:loki, fouladi:salsify, schwarz:svc-overview}, rate-adaptation algorithms~\cite{carlucci:google-cc, decicco:cc-for-webrtc, engelbart:cc-for-real-time-over-quic, rfc8698}, measurement studies to analyze meeting quality~\cite{bronzino:inferring-video-quality,michel:passive-measurement-zoom, chang:can-you-see-me, macmillan:perf-video-conferencing}, and network protocols~\cite{janczukowicz:specialized-net-servies-webrtc, elmokashfi:geography-matters}.

Though effective, existing work has primarily focused on the end user and network operator perspectives, with the challenges facing operators of VCA applications (and infrastructure) being far less explored. For VCA operators, the backbone of their applications are selective forwarding units (SFUs) that relay real-time audio and video traffic among meeting participants~\cite{gouaillard:webrtc-sfu-load-test,jitsi-videobridge,mediasoup,lopez:kurento}. Beyond relaying, these servers are also tasked with monitoring video and audio quality, and rapidly adapting media signals to match the time-varying network and compute capabilities of meeting participants during calls. To provide this degree of control, SFUs are typically implemented in user-space software on general-purpose CPUs. However, this flexibility comes at the cost of scalability (\S\ref{sec:dissect}) -- one that will only worsen as conferencing traffic continues to surge~\cite{feldmann:lockdown-effect, video-conf-market}. SFU operations involve forwarding many small UDP packets (for audio streams and feedback messages), an ill-suited task for operating systems~\cite{cai:understanding-lxovhs}. Plus, an SFU must be amenable to rapid shifts in resource overheads, which scale quadratically with the number of participants in a call, and also based on user behaviors such as enabling and disabling video/audio sharing during a call. %To provide this level of logic and control, SFUs are implemented in user-space software on general-purpose CPUs. However, this comes at the cost of efficiency, as VCAs generate thousands of (small) UDP packets that in short time periods that are ill-suited for forwarding with OSes

In this paper, we eschew pursuing ephemeral improvements to existing SFU mechanisms for scalability (e.g., improved software packet processing or provisioning mechanisms) in favor of a fundamental rethink of VCA infrastructure that can support long-term traffic forecasts. Guided by our detailed characterization of Zoom's SFUs (and a study of real Zoom campus traces  -- \S\ref{sec:dissect}), our key insight is that the forwarding and adapting of media signals at SFU servers is strikingly similar to traditional packet-processing tasks. For example, relaying a media stream to multiple participants is achieved by replicating and forwarding packets to different destinations; similarly, bitrate adaptation can be achieved by simply dropping specific subsets of a media stream's packets~\cite{schwarz:svc-overview}.


%Motivated by the sustained surges in conferencing traffic around the globe~\cite{feldmann:lockdown-effect, video-conf-market}, we eschew improvements to existing SFU mechanisms for scalability (e.g., better software packet processing or provisioning mechanisms) in favor of a fundamental rethink of VCA infrastructure. Guided by our detailed characterization of Zoom's SFUs (and a study of real Zoom campus traces), our key insight is that forwarding and adapting of media signals at SFU servers is strikingly similar to traditional packet processing tasks. For example, relaying a media stream to multiple participants is achieved by replicating and forwarding packets to different destinations; similarly, bitrate adaptation can be achieved by simply dropping specific subsets of a media stream's packets~\cite{!!!}.

Fueled by this insight, we present \textbf{\sys{}}, a software-defined networking (SDN)-inspired WebRTC SFU design and system that decouples VCA infrastructure into (1) an efficient data plane that relays media packets using line-rate network switching hardware, and (2) a software control plane that handles the remaining, \emph{infrequent} tasks (e.g., signaling, quality monitoring, congestion control, and connection setup). Realizing this vision with existing real-time multimedia protocols and constrained line-rate network devices poses numerous challenges, described in turn.

First, in order to introduce hardware-amenable SFUs, we need to depart from the way a WebRTC SFU, today, would be implemented which is leveraging a split-proxy design due to WebRTC's inherent design as a P2P application.
This implies terminating the connection, re-encrypting and re-packetizing media signals which not only in general is costly but most importantly cannot be implemented in a line-rate data-plane device.
Instead, in our design which is akin to a traditional proxy, we use unconventional ways of using the WebRTC APIs to split media connections across transport-layer streams and control signaling such that WebRTC selective forwarding can translate to match/action rules and feedback signals are handled correctly and consistently through the intermediate device.
Based on this, we went further and dissected WebRTC to enable an SDN-inspired control/data-plane split where media traffic is handled exclusively in a high-performance, low-latency data plane.

% webrtc designed p2p
% existing sfus do split proxy to deal with this
% we cant: would require switch to do XYZ (which is not even compatible with switch capabilities)
% instead, we had to repackage existing mechanisms to avoid split proxy (and 1-2 sentences saying what that 'repackaging' actually means)


% exiting use split proxy (oss)
% existing do 
% but also we cannot
% has implications
% more on what unconventional ways are


% to support the required app-layer tasks in the data plane, we repurpose key networking primitives...


% there is a mismatch between the required app-level tasks and the available network primitives in the data plane (and the resource constraints they must respect). To cope with this, we introduce a slew of bridging mechanisms that repackage data plane operations without adding undue overheads. For example, ....
Second, there is a gap between the application-level tasks \sys{} needs to perform and the capabilities of network-level primitives natively offered by the data plane. To cope with this, we introduce a slew of mechanisms that repackage data-plane operations to offer semantically rich, application-layer capabilities without adding undue overhead, while respecting the resource constraints of the data plane. For example, we use flexible, recursive network header parsing to extract media-level/L7 semantics from the complex wire protocols which use deep and dynamic header formats. We also leverage the multicast engine to replicate incoming media streams to their receivers by dissecting meeting topologies into multi-layer multicast trees. We enable rate adaptation by dynamically pruning branches of these multicast trees, while maintaining transparency to receivers in the presence of network loss and reordering by rewriting sequence numbers using a streaming heuristic that guarantees uninterrupted media decoding. We deploy \sys{} on the most performant and therefore also most resource-constrained family of commodity packet processors (i.e.,  high-speed, programmable switches) which demonstrates the strength of our design and enables us to advance the limits of application-aware packet processing.
% why primitives not amenable in first place
% mismatch between core app tasks and core network primitives 

%\ravi{Para on WebRTC with proxy servers}
%- using webrtc in non P2P manner
%- rework WebRTC to function with split control/data plane (even though it is designed for P2P settings). new strategies to use peer connections that allow for an intermediate processor while keeping all media signals valid and feedback signals consistent.


%\ravi{Para on data plane challenges: }
%repurpose core network functionality and use them to implement %application-layer tasks/semantics
%- dissecting protocols to split across hardware/software 
%- parsing
%- remaining transparent

%[don't want to do split connection and terminate at SFU.]
%- data plane challenges primarily center on resource constraints?
%\end{comment}

We implemented \sys{} using P4~\cite{bosshart:p4} on a 3.2 Tbit/s Intel Tofino ASIC~\cite{intel:tofino}. In experiments replaying campus-scale Zoom traces, we observe that \sys{}'s data and control split results in 96\% of video conferencing packets (and 99\% of overall bytes) being processed \emph{entirely} in hardware. Importantly, synchronous processing of media packets is exclusively handled in the data plane. Consequently, \sys{} can support up to 65,536 concurrent meeting participants on a single switch, an improvement of 20-40$\times$ over a 32-core commodity server, while avoiding software-processing artifacts on key performance metrics such as jitter that have direct impact on meeting quality by increasing the sizes of jitter buffers or causing stalls. 
% \ravi{@Oliver - you could add a sentence here about how we hope the primitives we introduce generalize to other in-network app tasks}
We believe that the video-conferencing constructs implemented by repackaging native network-level primitives can generalize to other in-network application tasks (see \S~\ref{sec:data}).
We will release the source code of \sys{} post publication.






==> sec/archive/related.tex <==
% !TEX root =  ../p4-sfu-nsdi24.tex

\section{Related Work}%
\label{sec:related}

\noindent
\textbf{Studies on video-conferencing applications.}
Baset and Schulzrinne's analysis of Skype, a famous P2P VoIP application in 2003~\cite{baset:analysis-of-skype}, provided crucial insights about Real-Time Communication (RTC) systems.
Nisticò et al. did a comprehensive and comparative study of different RTC applications~\cite{nistico:comparative-study-rtc}. Lee et al. did an in-depth measurement study 
on rate control algorithms used in popular commercial video-conferencing applications~\cite{lee:demystifying-vca}.
Two recent papers conducted extensive measurement studies of different video-conference applications such as Zoom, Meet, Teams, and WebEx~\cite{chang:can-you-see-me,macmillan:perf-video-conferencing}. Both studies shed light on the infrastructure, geographic location, lag, latency, bit rate, network utilization, and their impact on user Quality of Experience (QoE). Choi et al. did a more longitudinal and microscopic analysis of Zoom~\cite{choi:zoom-session-quality}.  Michel et al. did an in-depth study of Zoom traffic in a production network, demystifying the Zoom RTP packet format~\cite{michel:passive-measurement-zoom}. \\
%Bronzino et al. proposed a system where a trained AI/ML model can infer the quality of the video traffic  \cite{bronzino:inferring-video-quality}
%
\noindent
\textbf{Handling video-conferencing traffic in the data plane.}
Elmokashfi et al. presented the idea of creating an overlay IP network
on the Internet, just for video conferencing traffic. This work proposes a unique geo-based
BGP routing protocol, which performs ``cold-potato routing'' using GeoIP data~\cite{elmokashfi:geography-matters}. However, this work's approach is through geo-friendly routing, a control plane-based improvement. Data plane-assisted video conference traffic processing has been explored, but not extensively. Edwards and Ciarleglio showcased a programmable data plane 
that can parse, process, and produce ``clean'' video switching of uncompressed HD video flows based on the RTP timestamp~\cite{edwards:ts-aware-rtp-switch-p4}. The system was originally developed in the P4 language and later ported to the Cavium XPliant network processor. However, this demo focuses more on showing the capability of parsing RTP headers and making forwarding decisions based on RTP timestamp values with real hardware, rather than offloading any application-layer functionality (like an SFU).
More recent work showed that programmable data planes and eBPF/XDP programs running on servers can help with the NAT traversal functionality in video-conferencing applications~\cite{kfoury:offload-media-prog-switches,levai:supercharge-webrtc}. Both solutions offload the NAT traversal functionality, which is a heavy packet-processing workload, to a programmable data plane (e.g., Intel Tofino)~\cite{kfoury:offload-media-prog-switches} or an eBPF/XDP program~\cite{levai:supercharge-webrtc}. Our work goes way beyond this. Our work enables the data plane to also perform packet replication and selective forwarding of actual RTP media traffic, offloading such tasks from the server CPU. 

==> sec/archive/scale.tex <==
% !TEX root = ../p4-sfu-nsdi24.tex  

\section{Scaling Challenges of Video-Conferencing Infrastructure}
\label{sec:scale}

To provide background, understand the scalability properties of video-conferencing infrastructure, and to demonstrate the effects of under-provisioning selective forwarding units, in this section, we present a measurement study of Zoom~\cite{zoom} on our campus.
Our data includes higher-level usage statistics collected \textcolor{red}{over the course of ten days}, packet-level traces of Zoom traffic, as well as fine-grained VCA performance statistics gathered from controlled experiments using the MediaSoup open-source SFU~\cite{mediasoup}.
Before presenting our findings, we first provide background on video conferencing and SFUs.

\subsection{Background}
\label{ssec:background}

\textbf{Media Delivery in Video Conferencing.}~%
Besides connection establishment and signaling which is typically realized through protocols like the Session Description Protocol (SDP)~\cite{sdp-rfc} and Interactive Connectivity Establishment (ICE)~\cite{ice-rfc}, the key task of a video-conferencing application is to deliver media streams between meeting participants.
The protocol used for this is typically the Real-Time Protocol (RTP)~\cite{rtp-rfc}.
RTP is usually carried over UDP.
At the sender side, a media signal is generated by the camera or microphone.
This signal is then digitized, encoded, and packetized before sending over the network.
Typical codecs used in video conferencing include H.264~\cite{wiegand:avc} and recently AV1~\cite{av1} for video and Opus~\cite{opus-rfc} for audio.
The packetizer operates on a frame for video and a chunk of audio samples for audio.
A frame or sample may fit in a single packet but is more often spread over several RTP packets which are subsequently sent over the network.
At the receiver, the packets are received, depacketized, and decoded before being rendered on the screen or played through the speakers.
RTP's companion protocol the RTP Control Protocol (RTCP) is used to send feedback about the received packets, such as receive jitter and loss rate back to the sender where this information is fed into a rate controller.

% \textcolor{red}{TODO: short background on protocols used in media deliver, e.g., flow from sender, encoder, packetizer, to RTP packets over the network, mention encrypted payload but headers in the clear, also mention that sender performs rate selection and adaptation in conjunction with encoder, feedback signal through RTCP, etc.}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{fig/call-arch.pdf}
    \caption{Video-Conferencing Architectures: Peer-To-Peer (P2P) vs. Selective Forwarding (SFU). Each Color Represents a Participant's Media Stream.}
    \label{fig:call-arch}
\end{figure}

\noindent
\textbf{Meeting Topologies.}~%
Traditionally, Internet telephony and video-conferencing applications have been based on a peer-to-peer (P2P) architecture where each participant sends and receives media streams to and from every other participant~\cite{baset:analysis-of-skype}.
Direct P2P connections between meeting participants result in the lowest latency between two given clients but can be challenging to realize in the presence of firewalls and network address translators (NAT)~\cite{ice-rfc,ford:p2p-across-nat}.
The left side of Figure~\ref{fig:call-arch} depicts the media streams in a three-party P2P meeting.
Large P2P meetings put significant load on each sender as different versions of the media must be encoded to match different receiving participant's device and network capabilities (as illustrated by the dashed lines).
Moreover, as each sender sends an individual media stream per other participant, this approach requires substantial uplink bandwidth which is often not available in residential and wireless Internet access settings.
As a result, most VCAs use P2P connections only for some two-party calls (e.g., Zoom) or not at all (e.g., Google Meet)~\cite{nistico:comparative-study-rtc, michel:passive-measurement-zoom, lee:demystifying-vca}.

\noindent
\textbf{The Need for Scalable Forwarding Units.}~%
To avoid the uplink bottleneck problem, intermediate servers were introduced that forward media streams among clients.
These servers are called Selective Forwarding Units (SFU) and are the de-facto standard in video conferencing today.
Similar intermediate servers are used for live-streaming use cases~\cite{whip-whep-live-streaming}.
The topology in terms of media streams of a three-party SFU-based meeting is depicted on the right side of Figure~\ref{fig:call-arch}.
A SFU receives each client's media streams, replicates the streams for each downlink participant and forwards the media accordingly.
% This approach reduces the amount of uplink bandwidth required at the clients but, depending on the location of the SFU relative to the meeting participants, may significantly increase delay.
In addition to forwarding media, SFUs must adapt media streams for the network conditions, device capabilities, or preferences of individual downstream meeting participants.

\subsection{Provisioning SFUs is Hard}
\label{ssec:provisioning-sfus}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.98\columnwidth]{fig/participants-over-time-1}
%     \caption{Concurrent meeting participants over time. \textcolor{red}{note: time in UTC}}
%     \label{fig:part-over-time}
% \end{figure}

\noindent
We will now lay out the scaling challenges that arise when provisioning video-conferencing infrastructure.

\noindent
\textbf{Dynamic Workload.}~%
Like many user-facing services, video conferencing is subject to significant diurnal and weekly variations in usage.
Figure~\ref{fig:part-over-time} shows the number of concurrent meeting participants in Zoom meetings hosted by user accounts associated with our institution over the course of \textcolor{red}{ten days}.
As expected, we see significant peaks in workload during the working hours.
Apart from these variations, a second challenge stems from the dynamics within a given meeting.
The size of a meeting in terms of participants and their activity (resulting in media streams) is (1) often not predictable and (2) highly dynamic in nature.
% While the number of participants invited to a scheduled meeting might give an estimate for the number of participants, this data is often not available and is also not a reliable indicator for how these participants will behave in the meeting in terms of what media they share for how long and at what times.

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.48\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/part-duration-1}
        \caption{Join/leave duration.}
        \label{fig:part-duration}
    \end{subfigure}
    \hspace{0.01\columnwidth}
    \begin{subfigure}{0.48\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/sharing-frac-type-cdf-1}
        \caption{Media sharing duration.}
        \label{fig:sharing-frac-type-cdf}
    \end{subfigure}
    \caption{Participant activity within a meeting.}
\end{figure}

The problems that arise from the dynamic nature of video-conferencing meetings are twofold.
First, meeting participants do not necessarily all join at the same time around the beginning of the meeting and stay in the meeting for its entire duration.
Figure~\ref{fig:part-duration} depicts the distribution of the fraction of the total meeting duration that individual participants are present in a meeting.
We can see that only 25\% of users join a given meeting for (or close to) its entire duration.
Second, and even more importantly, it is rare that meeting participants share both of the two main media types (audio and video) for the entire duration of the meeting.
Figure~\ref{fig:sharing-frac-type-cdf} shows the distribution of the relative duration of each shared media type (audio, video, and screen) as a fraction of the user's presence in the meeting for each user in our data set broken down by media type.
For audio and video, we can see that only 50\% of users share their audio and video for more than 90\% of the time they are present in the meeting, resulting in frequent changes in the number of media streams that the SFU has to forward.

% \subsubsection{Quadratic Scaling}

\noindent
\textbf{Quadratic Scaling.}~%
While the use of SFUs solves the problem of constrained uplink bandwidth and reduces the required CPU resources at clients, SFUs do not entirely solve the scalability problem in multi-party video conferencing as sometimes suggested~\cite{webrtc-arch-basics-blog}.
It is important to note that the number of streams that are required in a SFU scenario still grows quadratically with the number of participants.
There are $N^2$ media streams for $N$ participants (per media type in use) in a SFU topology which even grows slightly faster compared to the $N(N-1)/2$ streams in a P2P topology (see Figure~\ref{fig:call-arch}).
The key difference is that all these streams are now sent to or received by the SFU, effectively moving the bottleneck from the clients to the SFU.

The second important observation is that the amount of work that a SFU needs to perform is determined by the number of streams and not by the number of participants which therefore leads to a quadratic scaling behavior at the SFU.
This is due to the fact that every incoming stream needs to be replicated for each of the downstream participants and then sent out accordingly (see Figure~\ref{fig:sfu-operation}).
At hundreds of packets (typically between 800 and 1400 Bytes in size for video and around 200 Bytes in size for audio) per second per stream, this requires copying significant amounts of data among socket buffers for receiving packets and before sending them out, resulting in high CPU load and frequent context switches.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\columnwidth]{fig/n-sfu-streams-1}
    \caption{Media streams that the SFU has to receive or send per meeting for different meeting sizes in campus dataset.}
    \label{fig:n-sfu-streams}
\end{figure}

% The SFU forwarding mechanism is illustrated in Figure~\ref{fig:sfu-operation}.
% Here, the SFU relays a media stream in a four-party meeting where each incoming packet needs to be replicated and per-stream adaptation logic needs to be applied.
% In this case, one of the participants receives a lower frame-rate stream which SVC enables by dropping every other frame.
% The scalability layers are here denoted by letters A and B and the inter-frame dependencies are depicted as arrows.

Of course and as noted above, not in every meeting every participant sends media to every other participant at all times.
We analyzed the number of media streams that Zoom's SFUs need to forward for each meeting on our campus as a function of meeting participants.
A media stream is counted as soon as it was active for at least 10\% of the meeting's duration.
Figure~\ref{fig:n-sfu-streams} shows the result of this analysis.
The error bars show the minimum and maximum number of streams seen in meetings of the respective size while the blue line corresponds to the median.
The dashed line indicates the upper bound of streams possible if every participant would share both audio and video.
We can see that even for meetings with 10 participants, the SFUs already handles up to 200 media streams.
Meetings with 25 participants, a typical classroom size, generate in excess of 600 media streams at the SFU in our data set and can theoretically produce up to 1200 streams.




% To show that the work a SFU has to perform grows with the number of streams rather than the number of participants, we conducted a simple experiment using Mediasoup~\cite{mediasoup}, a popular SFU implementation.
% We run a Mediasoup server on an AWS EC2 \textcolor{red}{xyz (size)} node and gradually increase the number of participants in a meeting (which join from other nodes) while monitoring the CPU utilization of the virtual machine.
% The result of this experiment is shown in Figure~\ref{fig:sfu-cpu-util}.
% We can see that the CPU utilization grows exponentially and approaches 100\% at roughly \textcolor{red}{X} participants.
% In Section~\ref{ssec:effect-underprovisioning}, we show how high CPU utilization of a SFU server directly affects the quality of the meeting as experienced by the clients.

% \textcolor{red}{\textit{OM: perhaps show no. of sys calls and sys. CPU as a function of no. of participants (seems more tangible than noisy CPU util. Also, just show for large meeting, e.g., 50 participants to prove the point, acknowledge that not every meeting is of that size
% }}

\subsection{Under-Provisioning Impairs QoE}
\label{ssec:effect-underprovisioning}

To demonstrate the consequences of under-provisioning video-conferencing infrastructure, we conducted a controlled experiment using the popular Mediasoup open-source SFU~\cite{mediasoup}.

\noindent
\textbf{Experiment Setup.}~%
We ran the Mediasoup demo application~\cite{mediasoup-demo} on a server with a 40-core Intel Xeon Silver 4114 CPU clocked at 2.20GHz and 96GB of RAM.
A second server with similar characteristics emulated clients using headless Chrome.
Both servers are located in the same rack and are connected through a \textcolor{red}{1Gbit/s} Ethernet connection.
To run the experiment, we pin the Mediasoup server to a single CPU and emulate 15 meetings with 10 participants each.
We gradually added one participant every ten seconds.
During the experiment we measured the CPU utilization of the Mediasoup server as well as the quality of the meeting as experienced by the first client of the first meeting using the statistics available through the WebRTC statistics API~\cite{webrtc-stats}.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.75\columnwidth]{fig/cpu-part-1}
%     \caption{CPU Utilization as we add participants to a Mediasoup session.}
%     \label{fig:cpu-part}
% \end{figure}

% \noindent
% \textbf{Mediasoup CPU Utilization.}~%
% Figure~\ref{fig:cpu-part} shows the mean CPU utilization of the Mediasoup server as we add participants to the meetings.
% While we can see some slight exponential growth within the first two meetings (1-20 participants), the curve starts to flatten as we hit higher CPU utilization.
% At around 80-100 participants, we reach 90-100\% CPU utilization.
% \textcolor{red}{TODO: add more details about CPU utilization, e.g., syscalls, etc.}

\begin{figure*}[t]
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{fig/mean-video-rx-rate-1}
        \caption{Video Receive Rate}
        \label{fig:mean-video-rx-rate}
    \end{subfigure}
    \hspace{0.35cm}
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{fig/video-rx-jitter-1}
        \caption{Video Receive Jitter}
        \label{fig:video-rx-jitter}
    \end{subfigure}
    \hspace{0.35cm}
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{fig/rx-fps-1}
        \caption{Video Frame Rate}
        \label{fig:rx-fps}
    \end{subfigure}
    \caption{QoS metrics gathered through the WebRTC statistics API for the first client of the first meeting.}
    \label{fig:que-degradation}
\end{figure*}

\noindent
\textbf{QoE Degradation.}~%
Video-conferencing is a real-time application where the perceived quality of the meeting is mostly determined by the receiver's ability to decode and render a high-quality media stream without incurring excessive mouth-to-ear delay (e.g., by using a large receiver buffer to compensate for jitter and loss).
To quantify the quality of the meeting as experienced by the first client of the first meeting, we use QoS data available through the WebRTC statistics API which reports various media- and network-related metrics from the receiver's and media decoder's perspective~\cite{webrtc-stats}.
Figure~\ref{fig:que-degradation} shows three key metrics from the perspective of the first participant of the first meeting as we start meetings and add participants one by one.

It is important to note that the configuration of the individual meetings stays the same as soon as all ten participants have joined.
Consequently, any changes in quality of the first meeting past the tenth participant are not due to the configuration of the meeting but rather due to the increased load at the SFU.
During our experiment, the SFU server reached 100\% CPU utilization at around 80-100 participants.
Figure~\ref{fig:mean-video-rx-rate} shows the mean video receive rate over time.
We can see that the rate drops significantly with higher workload at the SFU, even below 300 kbit/s where the video (visual) quality is likely heavily impaired.

Being a real-time application video conferencing is particularly sensitive to delay and jitter.
Figure~\ref{fig:video-rx-jitter} shows the receive jitter measured in millisecond.
Starting at 125 participants, the tail jitter exceeds 100ms which either results in significant mouth-to-ear delay compromising the interactivity of the meeting due to a large jitter buffer or causes periodic freezes.
Given that the SFU and client machine were connected to each other via a \textcolor{red}{1 Gbit/s} directly-attached Ethernet link, it is unlikely that the jitters stems from the network but rather from resource contention at the SFU.

Finally, Figure~\ref{fig:rx-fps} shows the frame rate of the received video stream.
Similar to the receive rate, we can see that the frame rate drops significantly with higher workload at the SFU.
Beyond 60 participants, we see increasingly frequent frame-rate drops with the frame rate dropping below five beyond 130 participants which means frequent picture freezes for the participant.
We conclude that overloading the SFU has direct and noticeable consequences for the quality of the meeting as experienced by the participants; this extends to the point where the meeting becomes effectively unusable (in our case from around 120 participants on).
